Studies on Coupled Flight Dynamics and Aeroelasticity of a Prandtlplane Configuration

The PrandtlPlane aircraft has been recently considered as a possible candidate to foster the ambition of a greener aviation. Despite the relevant amount of research carried out in the last years, several aspects of this novel configuration still need further insight to pave the way to future applications. Among them, the coupled flight-dynamic and aeroelastic response is addressed in this work by means of a dedicated in-house framework. For the evaluation of the aerodynamic forces, an enhanced Doublet Lattice Method, able to take into account terms typically neglected by classic formulations, is employed. First, flight-dynamic aspects are considered, showing how effects of interaction between Short Period or Dutch Roll with elastic modes remarkably deteriorate the flying qualities. Then, focus is on the aeroelastic stability of the aircraft. As observed also in previous literature efforts on this configuration, flutter onset is considerably different when considering the aircraft being free in the air or fixed in space. Thanks to the adopted formulation it is shown how, for this PrandtlPlane, the aerodynamic coupling of elastic and rigid modes has a beneficial effect on flutter onset. However, the different modal properties, consequence of the diverse boundary conditions, when switching from fixed-in-space to free-flying aircraft, also play a relevant role in determining the occurrence of flutter. Whereas for the longitudinal case both effects contribute increasing flutter speed, for the lateral-directional case the variation in modal properties has a detrimental and dominating effect, leading to a flutter speedwell within the flight envelope.Finally,the work discusses the contributions of the additional terms modeled by the enhanced Doublet Lattice Method, showing how they induce a considerable effect when modeling the flight dynamics of the flexible aircraft.

==> chapters/Acknowledgments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555
\section{Acknowledgments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Part of this research, i.e., the development of the structural finite element capabilities as well as the interface/splining to transfer loads/displacements between the structural and aerodynamic grids has been supported by grant DPI2016-76151-C2-2-R (AEI/FEDER, UE).



%This , \inred{currently under development for a funded research by the Spanish government}. 

==> chapters/IFAS_chapII.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  %
\subsection{Kinematics and
Reference Systems}   %
%                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In general we consider two different reference frames: an inertial one $\left( \Sigma_I \right) $ and a body (vehicle-fixed) one $\left( \Sigma_B \right) $.
The inertial position $\bR$ of a material point P (of infinitesimal volume $\ddi V$) can be expressed in terms of the inertial position of the origin of the body frame $\bR_{O_B}$, plus the relative position of the mass element in the body frame $\br$, as depicted in Fig.~\ref{fig:inertial_vehicle_frames}.
% in which the inertial (Frame I) and the body (Frame B) frames are shown
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bR=\bR_{O_B}+\br\end{aligned}
\label{eq:pos}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%

%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
\centering
          \includegraphics[width=0.8\textwidth]{../figures/References_General}
  \caption{Inertial and body frames and position vectors}
  \label{fig:inertial_vehicle_frames}
\end{figure}
%----------------------------|
%
Its inertial velocity is
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bV_{P}= \bV = \left. \frac{\ud \bR}{\ud t} \right|_I = \underbrace{\left. \frac{\ud \bR_{O_B}}{\ud t} \right|_I}_{\bV_{O_B}} + \left. \frac{\ud \br}{\ud t} \right|_I
\end{aligned}
\label{eq:in_velocity_element}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $\bV_{O_B}$
%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%\frac{\ud \bR_{O_B}}{\ud t}{\big |}_I = \bV_{O_B}
%\end{aligned}
%\label{eq:in_velocity_V}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
is the inertial velocity of the origin of body-frame $\Sigma_B$.
The last term, the inertial velocity of a point in the body reference frame, can be further expanded
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\left. \frac{\ud \br}{\ud t} \right|_I = \left. \frac{\ud \br}{\ud t} \right|_B+\bom_{B,I}\x\br
\end{aligned}
\label{eq:in_velocity_p}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
with $\bom_{B,I}$ angular velocity of $\Sigma_B$ with respect to  $\Sigma_I$, and $ \left. \frac{\ud \br}{\ud t} \right|_B$ the relative velocity as seen from $\Sigma_B$. %, convenientely expressed using Poisson's formula.
%
The relative velocity can be further transformed expressing the position $\br$ of a generic material point $P$ %(with respect to the origin $O_B$)
as the initial/reference position $\br_{o}$ plus a variation $\bu\left(x,y,z; t\right)$:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\br=\br_{o}+\bu\left(x,y,z,t\right)
\end{aligned}
\label{eq:RB+def}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Thus the relative velocity can be expressed as
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\dot{\br} = \left. \frac{\ud \br}{\ud t} \right|_B = \left. \frac{\ud \bu}{\ud t} \right|_B  = \dot{\bu}
\end{aligned}
\label{eq:pos_derivative}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
since the vector $\br_{o}$ is invariant with respect to Frame B.
%
Therefore, the inertial velocity is:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bV = \bV_{O_B}+\bom_{B,I} \x \br +\dot{\br}= \bV_{O_B}+\bom_{B,I} \x \left(\br_{o}+\bu \right)+\dot{\bu}
\end{aligned}
\label{eq:in_velocity_final}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Notice that, at this point, $\bu$ cannot be uniquely associated to deformations due to structures elasticity as the body-fixed system has not been yet defined.
%
%**********************************%
%                                  %
\subsection{The \emph{Mean Axes}
                          Frame}   %
%                                  %
%**********************************%
%
Although the choice of the frame in which describes the flight dynamic of the vehicle is arbitrary, the equations governing the dynamics of the flexible aircraft can be simplified with an ad-hoc choice of the vehicle-fixed frame.
In references~\cite{Milne1962,Milne1968} it is noted that for an elastic body always exists a coordinate frame such that the relative linear and angular momenta, due to elastic deformation, are zero at every instant.
This noninertial reference system is called \emph{mean axes} frame and its origin coincides with the instantaneous center of mass of the vehicle.
These axes move in phase with the body motion but they are not attached to any fixed point in the aircraft.
%
\par
%
From the definition we obtain the \emph{mean-axes} constraints (or properties):
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\left\{
\begin{aligned}
&\int_{\text{Vol}} \left. \frac{\ud \br}{\ud t} \right|_B \rho_\text{V}\ud\text{V} =  \bzero \\
&\int_{\text{Vol}} \br \x \left. \frac{\ud \br}{\ud t} \right|_B \rho_\text{V}\ud\text{V} = \bzero
\end{aligned}
\right.
\label{eq:mean_axes}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $\rho_\text{V}$ is the density of the material, and $\int_{\text{Vol}}$ represents the integral over the aircraft; considering eqs.~(\ref{eq:RB+def}) and (\ref{eq:pos_derivative}), we obtain:
% the \emph{practical mean-axes constraints}
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\left\{
\begin{aligned}
&\int_{\text{Vol}} \left. \frac{\ud \bu}{\ud t} \right|_B \rho_\text{V}\ud\text{V} =  \bzero \\
&\int_{\text{Vol}} \br_{o} \x \left. \frac{\ud \bu}{\ud t} \right|_B \rho_\text{V}\ud\text{V}+\int_{\text{Vol}} \bu \x \left. \frac{\ud \bu}{\ud t} \right|_B \rho_\text{V}\ud\text{V} = \bzero
\end{aligned}
\right.
\label{eq:mean_axes_practical1}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
\newtheorem{remark}{Remark}
\begin{remark}
It is generally not true that $\bu \neq \bzero$ only if there are deformations (intended as change in the shape of the aircraft): for example, burned fuel can change the location of the $CoM$, and thus, $\bu \neq \bzero$ even though the shape of the aircraft is coincident with the initial/reference one.
From now on, however, $\bu$ will be associated to deformations (change of the shape of the aircraft).
\end{remark}
%
%
%*****************************************
\subsubsection{Structural displacements}
%*****************************************
Here and for the rest of the paper, the hypothesis of ``linear'' behavior of the structure is assumed; other than linear elastic material, deformations/strains are small, and linear kinematic relation between the displacements and the strain holds. Moreover, the equilibrium of the internal structural forces is enforced on the undeformed/reference configuration.
%
\par
%
In structural dynamics engineering, it has been observed that  projection of the structural displacements onto normal modes basis leads to convergence with a reduced number of modes.
For this reason, it is possible to retain the physical properties of the system with a very reduced number of modes.
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\bu(x,y,z; t) = \sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right){\eta}_i\left(t\right)
\label{eq:modal_decomp}
\end{equation}
%
where $\boldsymbol{\nu}_i$ represents the generic $i$th normal mode, and ${\eta}_i$ the relative coefficient.
%
%*****************************************
\subsubsection{Mean Axes constraint for small displacements}
%*****************************************
%
With the hypothesis of small displacements, the third integral in eq.~(\ref{eq:mean_axes_practical1}) is negligible, thus, the constraint reads:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\left\{
\begin{aligned}
&\int_{\text{Vol}} \left. \frac{\ud \bu}{\ud t} \right|_B \rho_\text{V}\ud\text{V} =  \bzero \\
&\int_{\text{Vol}} \br_{o} \x \left. \frac{\ud \bu}{\ud t} \right|_B \rho_\text{V}\ud\text{V} = \bzero
\end{aligned}
\right.
\label{eq:mean_axes_practical2}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%
The first term of eq.~(\ref{eq:mean_axes_practical2}) can be further expanded, using a $n$th dimensional normal modes basis:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\int_{\text{Vol}} \left. \frac{\ud \bu}{\ud t} \right|_V \rho_\text{V}\ud\text{V} =
\int_{\text{Vol}} \sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right)\dot{\eta}_i\left(t\right)\rho_\text{V}\ud\text{V}=
\sum_{i=1}^n \dot{\eta}_i\left(t\right) \left(\int_{\text{Vol}}  \boldsymbol{\nu}_i\left(x,y,z\right)\rho_\text{V}\ud\text{V}\right)=
\bzero
\end{aligned}
\label{eq:mean_axes_practical3}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
and we find that each term in parenthesis will be zero if the modal orthogonality among the vibration modes and the rigid-body translation ones is guaranteed. SONO QUI. DENTRO INTEGRALE?
Likewise, for the second term of eq.~(\ref{eq:mean_axes_practical2}) we find that
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\int_{\text{Vol}} \br_{o} \x \left. \frac{\ud \bu}{\ud t} \right|_V \rho_\text{V}\ud\text{V} =
\sum_{i=1}^n \dot{\eta}_i\left(t\right) \left(\int_{\text{Vol}}  \br_{o} \x \boldsymbol{\nu}_i\left(x,y,z\right)\rho_\text{V}\ud\text{V}\right)=
\bzero
\end{aligned}
\label{eq:mean_axes_practical4}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
and so that every term in parentheses is zero if the vibration modes are orthogonal to the rigid-body rotation ones (see reference~\cite{Canavin1977} for an alternative proof of the same properties).
So the mean-axes practical constraints can be interpreted as requiring the orthogonality among all the modes; the mean axes frame can clearly be found by satisfying this property.
%
[rivedere questa parte con ortognalità. Fra l'altro non capisco se è una causa o un effetto].
%
\par
%
In \cite{Canavin1977} is shown that this set of axes is the one that provides the minimum kinetic energy relative to the floating frame.
It is also demonstrated that in order to satisfy the mean-axes constraints the rigid modal coordinates must be zero: in other words, this frame chases the rigid-body motion and we can properly separate the elastic deformation effects.[ ????]
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  %
\subsection{Lagrange's Equation}   %
%                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Lagrange's equation states:
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\frac{\ud}{\ud t}\left(\frac{\pd T}{\pd \dot{\mbbm{q}}}\right)-\frac{\pd T}{\pd {\bq}}+\frac{\pd U}{\pd \bq}=\bQ^{\rT}= \frac{\pd \left(\delta W\right)}{\pd \left(\delta{\bq}\right)}
\end{aligned}
\label{eq:lagrange}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
being:
%
%----------------
\begin{itemize}
%----------------
    \item[] $T:$ the system total kinetic energy;
    \item[] $U:$ the potential energy of the system, including the strain energy of the elastically deformed body;
    \item[] $\bq:$ the vector of generalized coordinates used to describe the system;
    \item[] $\bQ:$ the vector of generalized forces acting on the system;
    \item[] $\delta \bq:$ the vector of virtual displacements of the generalized coordinates;
    \item[] $\delta W:$ the virtual work done by external forces acting on the vehicle.
\end{itemize}
%----------------  END ITEMIZE
%
%
We will specialize each term of the above equation for the case of \emph{Mean Axes} frame.
%
%%
%**********************************%
%                                  %
\subsubsection{Kinetic Energy}     %
%                                  %
%**********************************%
%
Starting with the definition of kinetic energy, and using the mean-axes frame constraints [UNIFORMARE il nome di mean axes frame] one obtains:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{split}
T  = \frac{1}{2}m \left. \frac{\ud \bR_{O_B}}{\ud t}\right|_I  \cdot
\left. \frac{\ud \bR_{O_B}}{\ud t}\right|_I +
\frac{1}{2} \bom_{B,I}^{\rT}\left[\bI_o\right] \bom_{B,I}+
\frac{1}{2} \int_{\text{Vol}} \left. \frac{\ud \br}{\ud t}\right|_B
\cdot
\left. \frac{\ud \br}{\ud t}\right|_B \rho_\text{V}\ud\text{V}
\end{split}
\label{eq:T_mean_axes_final2}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $m$ is the total mass of the aircraft, $\bI_o$ the inertia tensor of the undeformed configuration (measured considering the body frame origin as pole).
%
\par
%
It is clear that the choice of the mean-axes frame has led to an inertial decoupling: the effects of rigid-body translations (first term of right-hand side), rigid-body rotations (second term of right-hand side) and elastic deformations are completely decoupled. More details are shown in reference~\cite{Schmidt2012}.
The last term in the kinetic energy expression eq.~(\ref{eq:T_mean_axes_final2}) can be rewritten using the eq.~(\ref{eq:modal_decomp}) as:

%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{split}
\int_\text{Vol} \left. \frac{\ud \br}{\ud t}\right|_B \cdot
\left. \frac{\ud \br}{\ud t}\right|_B \rho_\text{V}\ud\text{V} =
\int_\text{Vol} \left. \frac{\ud \bu}{\ud t}\right|_B
\cdot
\left. \frac{\ud \bu}{\ud t}\right|_B \rho_\text{V}\ud\text{V} =
\int_\text{Vol} \left(\sum_{i=1}^n \boldsymbol{\nu}_i\frac{\ud \eta_i}{\ud t} \cdot \sum_{i=1}^n \boldsymbol{\nu}_i\frac{\ud \eta_i}{\ud t}\right)\rho_\text{V}\ud\text{V}
%
\end{split}
\label{eq:T_mean_axes_de}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
but due to orthogonality of the free vibration modes [UNIFORMARE FREE VIBRATION AND NORMAL MODES] it can be further simplified. Since:
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{split}
%\int_\text{Vol} \boldsymbol{\nu}_i \cdot \boldsymbol{\nu}_j\rho_\text{V}\ud\text{V}=&\begin{cases}
%0 & i\neq j \\
%\bM_i& i=j
%\end{cases}
%\end{split}
%\label{eq:mod_ort}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{split}
& \int_\text{Vol} \boldsymbol{\nu}_i \cdot \boldsymbol{\nu}_j\rho_\text{V}\ud\text{V}= 0,~i\neq j\\
& \int_\text{Vol} \boldsymbol{\nu}_i \cdot \boldsymbol{\nu}_j\rho_\text{V}\ud\text{V}= \bM_i,~i=j
\end{split}
\label{eq:mod_ort}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
where $\bM_i$ is the generalized mass of the $i$th vibration mode. Thus,
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{split}
\int_\text{Vol} \left. \frac{\ud \br}{\ud t}\right|_B
\cdot
\left. \frac{\ud \br}{\ud t}\right|_B \rho_\text{V}\ud\text{V} =
\int_\text{Vol} \left(\sum_{i=1}^n \boldsymbol{\nu}_i \cdot  \boldsymbol{\nu}_i\left(\frac{\ud \eta_i}{\ud t}\right)^2\right)\rho_\text{V}\ud\text{V} =
\sum_{i=1}^n \bM_i \dot{\eta}_i^2
%
\end{split}
\label{eq:T_mean_axes_de2}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%**********************************%
%                                  %
\subsubsection{Potential Energy}   %
%                                  %
%**********************************%
%
The potential energy of the vehicle includes both gravitational potential energy $U_g$ and the elastic strain energy $U_e$.
%
The gravitational term is the integral of the potential energy of the mass elements, so if $\bg$ is the acceleration due to gravity
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
U_g = - \int_{\text{Vol}} \left(\bg \cdot \bR \right) \rho_\text{V}\ud\text{V}= - \int_{\text{Vol}} \left(\bg \cdot \left(\bR_{O_B}+\br\right)\right)\rho_\text{V}\ud\text{V}
\end{aligned}
\label{eq:gravitational_energy}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%%The elastic strain energy is the energy stored by the system undergoing deformations. Using D'Alambert's principle (\inrosso{how?, see \cite{Schmidt2012}}), the elastic strain energy is
%%%
%%%---------------------------------
%%% EQ                  |
%%%---------------------------------
%%\begin{equation}
%%\begin{aligned}
%%U_e = -\frac{1}{2} \int_{\text{Vol}}\left( \left.\frac{\ud^2 \bu}{\ud t^2}\right|_B \cdot \bu \right)\rho_\text{V}\ud\text{V}
%%\end{aligned}
%%\label{eq:strain_energy}
%%\end{equation}
%%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%%
%%
%%
%% \inblue{*}\inrosso{dubbio:l'origine si sposta in generale, quindi la distanza di uno stesso punto anche `` fermo'' cambia. Vuol dier che metto in $\bu$ anche questo contributo?SOLVED: per effetto deformazioni, il cg non si sposta, dunque ho effettivamente scisso i due contributi. Da analizzare caso massa variabile e non deformazioni (att. cambia matrice massa sistema, modi ecc... }).
%%

%The free-vibration modes can be used to rearrange the elastic strain energy in eq. \ref{eq:strain_energy}. Indeed, being
%%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{split}
%\frac{\ud^2 \bu}{\ud t^2}\right|_B = \sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right)\ddot{\eta}_i\left(t\right)
%\end{split}
%\label{eq:de_2}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%and invoking the orthogonality of the vibration modes
%%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%U_e = & -\frac{1}{2} \int_{\text{Vol}}\left(\frac{\ud^2 \bu}{\ud t^2}\right|_B \cdot \bu \right)\rho_\text{V}\ud\text{V} = \\
%= &- \frac{1}{2} \int_{\text{Vol}}\left(\sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right)\ddot{\eta}_i\left(t\right) \cdot \sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right){\eta}_i\left(t\right)\right)\rho_\text{V}\ud\text{V}= \\
%=& - \frac{1}{2} \int_{\text{Vol}}\left(\sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right) \cdot \boldsymbol{\nu}_i\left(x,y,z\right)\ddot{\eta}_i\left(t\right){\eta}_i\left(t\right)\right)\rho_\text{V}\ud\text{V}= \\
%=& \frac{1}{2} \sum_{i=1}^n \om_i^2\eta_i^2\left(t\right)\bM_i
%\end{aligned}
%\label{eq:strain_energy2}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%The last step was achieved remembering the time response form of each generalized coordinate and where $\om_i$ is the vibration frequency for the i'th mode.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  %
\subsection{Equation of motion
             in mean-axes frame}   %
%                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Now that the terms composing the Lagrange's equation have been determined, we can explicitate the equation of motion.
However, we must previously choose the Lagrangian (or generalized) coordinates.
%
%**************************************%
%                                      %
\subsubsection{Generalized coordinates}%
%                                      %
%**************************************%
%
Let's define the vehicle's inertial velocity (of its center of mass) as:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bV_{O_B} = \left.\frac{\ud \bR_{O_B}}{\ud t}\right|_I = \dot{R}_{O_{B_X}} \bi_I+ \dot{R}_{O_{B_Y}} \bj_I+ \dot{R}_{O_{B_Z}} \bk_I
\end{aligned}
\label{eq:intertial_V}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\
%
with $\bi_I$, $\bj_I$, $\bk_I$ the unit vectors in each of the coordinate directions of the inertial Frame I and ${R}_{O_{B_X}}$, ${R}_{O_{B_Y}}$, ${R}_{O_{B_Z}}$ the components of the inertial position.
%
\par
%
The inertial orientation of the body-reference (mean-axes) frame is described by the 3-2-1 Euler angles $\psi$, $\theta$, $\phi$ and their rates are related to the components of the angular velocity of Frame B with respect to the Frame I $\left(\bom_{B,I}=\left\{P,Q,R\right\}^{\rT} \textrm{expressed in the body frame} \right)$ by the following equations [TOGLIERE TRASPOSTA A TUTTI I VETTORI?]
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\left\{
\begin{aligned}
& \dot{\phi} = P +Q\sin{\phi}\tan{\theta}+R\cos{\phi}\tan{\theta}\\
& \dot{\theta} = Q\cos{\phi}-R\sin{\phi}\\
& \dot{\psi} = \left(Q\sin{\phi}+R\cos{\phi}\right)\sec{\theta}
\end{aligned}
\right.
\label{eq:euler}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
also, known as Euler equations.
%
\par
%
It is clear that the components of the inertial position and the Euler angles allow the description of the rigid-body degrees of freedom of the vehicle. Thus, adding the modal coordinates $\eta_i$ used to describe the deformation of the vehicle (see eq.~(\ref{eq:modal_decomp}) we obtain the set of generalized coordinates of the system:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bq=\left\{{R}_{O_{B_X}},~{R}_{O_{B_Y}},~{R}_{O_{B_Z}},~\phi,~\theta,~\psi,~\eta_i\right\}^{\rT}
\end{aligned}
\label{eq:generalized_coordinate}
\end{equation}
%
with $i=1,2,\cdots,n$ and being $n$ the number of vibration modes.
%
%
%**************************************%
%                                      %
\subsubsection{Rigid-body translation} %
%                                      %
%**************************************%
%
Let's apply Larange's equation assuming just the three generalized coordinates relative to the inertial position of the center of mass $\bR_{O_B}=\left\{{R}_{O_{B_X}},{R}_{O_{B_Y}},{R}_{O_{B_Z}}\right\}^{\rT}$
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\frac{\ud}{\ud t}\left(\frac{\pd T}{\pd \dot{\bR}_{O_B}}\right)-\frac{\pd T}{\pd {\bR_{O_B}}}+\frac{\pd U}{\pd \bR_{O_B}}=\bQ^{\rT}_{trasl}= \frac{\pd \left(\delta W\right)}{\pd \left(\delta{\bR_{O_B}}\right)}
\end{aligned}
\label{eq:lagrange_traslation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Therefore, the equation governing the translational rigid-body degrees of freedom is simply:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
&m \left(  \left.\frac{\ud \bV_{O_B}}{\ud t}\right|_B+\bom_{B,I} \x \bV_{O_B}\right)
=m \bg + \bQ^{\rT}_{trasl}\\
\end{aligned}
\label{eq:lagrange_translation3}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
It is worth to underline that  eq.~(\ref{eq:lagrange_translation3}) is identical to the one typically expected for a rigid body; the effects of elasticity are included in the aerodynamic forces on the right-hand sides, which are sensitive to elastic deformations.
%
%**************************************%
%                                      %
\subsubsection{Rigid-body rotation} %
%                                      %
%**************************************%
%
Defining:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bq_\measuredangle = \left\{\phi,\theta,\psi\right\}^{\rT}
\end{aligned}
\label{eq:coordinate_rotation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
as the collection of Euler angles and applying the Lagrange's equation to these portion of generalized coordinates we derive the equations of motion governing rigid-body rotations as shown in \cite{Schmidt2012}:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\frac{\ud}{\ud t}\left(\frac{\pd T}{\pd \dot{\bq}_\measuredangle}\right)-
\frac{\pd T}{\pd {\bq_\measuredangle}}+\frac{\pd U}{\pd \bq_\measuredangle}=\bQ_{rot}^{\rT}= \frac{\pd \left(\delta W\right)}{\pd \left(\delta{\bq_\measuredangle}\right)}
\end{aligned}
\label{eq:lagrange_rotation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Other than exploiting the mean-axes frame properties, we also consider negligible the variation of the inertia tensor due to deformations, obtaining then [DECIDERE NOTAZIONE PER MATRICI/TENSORI]:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\left[\bI_0\right]\dot{\bom}_{B,I}+{\bom}_{B,I}\x \left( \left[\bI_0\right] {\bom}_{B,I}\right) = \bQ_{rot}^{\rT}
\end{aligned}
\label{eq:eqom_rotation_vectorial}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
To obtain the equations above,  eqs.~(\ref{eq:euler}) have been used to relate the Euler's angles and the components of the angular velocity.
%
\par
%
As for the translational dynamics, effects of the deformable structure are introduced into this equation through the aerodynamic forces, namely, by $\bQ_{rot}^{\rT}$
which includes both rigid and elastic effects.
%
%**************************************%
%                                      %
\subsubsection{Elastic deformation}    %
%                                      %
%**************************************%
%
The equations of motion governing elastic deformation can be easily obtained starting from the relative Lagrange's equation.
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\frac{\ud}{\ud t}\left(\frac{\pd T}{\pd \dot{\eta}_i}\right)-\frac{\pd T}{\pd {\eta_i}}+\frac{\pd U}{\pd \eta_i}=Q_i= \frac{\pd \left(\delta W\right)}{\pd \left(\delta{\eta_i}\right)}
\end{aligned}
\label{eq:lagrange_deformation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
With the aid of the constraints introduced by the mean-axes frame, we can finally write:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\ddot{\eta}_i+\om_i^2\eta_i = \frac{Q_i}{M_i},~~ i=1,\dots,n
\end{aligned}
\label{eq:eom_deformation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $M_i$ is the generalized mass and $Q_i$ the generalized force, each associated with the $i$th free vibration mode.
%
The generalized forces may be determined from the Principle of Virtual Work introducing the local elastic virtual deformation:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\delta\bu = \sum_{i=1}^n \boldsymbol{\nu}_i\left(x,y,z\right)\delta\eta_i\left(t\right)
\end{aligned}
\label{eq:virtual_deformation}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%
\begin{remark}
It is possible to demonstrate that, with the choice of the mean-axes frame, only the elastic modes concur in describing the deformation displacement field $\bu$; the $\eta_i$ associated with rigid modes are identically null.
\end{remark}
%
%
%**************************************%
%                                      %
\subsubsection{Kinematic equations}    %
%                                      %
%**************************************%
%
Eqs.~(\ref{eq:lagrange_translation3}, \ref{eq:lagrange_rotation} augmented with the kinematic relation (\ref{eq:euler}) define the problem.
Practically, it is more convenient to work considering both the linear and angular velocities in the body reference frame.
Thus, we still need a relation between the time derivatives of the translational rigid generalized coordinates, and the velocity of the body reference frame expressed in the same  frame.
This is trivially done with the direction-cosine matrix $\mbbm{T}_{I-B}$, defined such that:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\left\{\begin{matrix}\dot{R}_{O_X}\\ \dot{R}_{O_Y}\\ \dot{R}_{O_Z}\end{matrix}\right\} = \bT_{I-B} \left\{\begin{matrix}U\\V\\ W\end{matrix}\right\}
\end{aligned}
\label{eq:kinematic1}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%

%\item an equation that relates the rates of Euler angles to the components of the angular velocity of Frame B with respect to the Frame I $\bom_{B,I}$ (eq. \ref{eq:euler}).
%\end{enumerate}
%
%
%%\inrosso{TO DO: 1) distinzione Tisserand Frame-Mean axes, vedi libro indiano ecc.}.
%
%
%% 

==> chapters/IIb_Theory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  %
\subsection{Aerodynamic Model}     %
%                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{ss:Aerodynamic}
%%
In this section the calculation of the aerodynamic forces by means of the enhanced DLM is presented and the integration in the framework for the study of stability is discussed.
%
\par
%
%\inblue{This section will tackle in-depth the evaluation of the aerodynamic forces by means of the a DLM~\cite{Rodden_1968,Rodden_Taylor_1998}, a widely-used approach in aeroelasticity.}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\inblue{[DA LEGGERE]} Enhanced Doublet Lattice Method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Study of the aeroelastic stability of the herein investigated PrandtlPlane configuration have been extensively pursued in the years, by the authors of the current effort, by means of an in-house aerodynamic force calculation module based on the DLM originally proposed by Rodden~\cite{Rodden_1968,Rodden_Taylor_1998}; a standard and still widely-used approach in aeroelastic analysis.
%
\par
%
It is known, though, that, in its original formulation, the DLM only calculates the unsteady aerodynamic loads and relative generalized forces due to pitching and plunging of the aerodynamic surfaces, ignoring the contribution of in-plane forces due to yawing and spanwise in-plane motions. Moreover, contribution to forces due to steady-state aerodynamic loads (i.e. loads due to the trim condition) are also ignored. 
%
\par
%
While the approximation is acceptable and delivers good results for the most of applications on conventional wings, it is demonstrated not to calculate all the necessary aerodynamic loads for flutter analysis of T-tails~\cite{VanZyl-2011}. In this case, both in-plane loads and normal loads due to in-plane motions are important to consider. Similarly, for a box-wing configuration as the PrandtlPlane, investigated in this effort, such contributions are important to take into account as it will be demonstrated in the following.
%
\par
%
The enhancement to the traditional DLM are included following efforts~\cite{VanZyl-2011,VanZyl-2008,Kier2011AnIL,Kier2009UNIFYINGMA} and consists in a more general boundary condition, to take into account yaw-dihedral coupling, and a forces calculation method that considers lateral loads and yawing moment due to roll rate and rolling moment due to yaw and yaw rate (particularly important when dealing with lateral-directional stability analysis).
%------------------------------------------%
% FIGURE    LOCKHEED                       %
%------------------------------------------%
\begin{figure}[htb]
     \centering
     \vspace{5mm}
         \includegraphics[width=\textwidth]{./figures/Enhanced_DLM}
         \caption{Enhanced DLM: unsteady boundary condition (a) and forces (b).\inred{Da rifare carina con AI}}
         \label{f:Enhanced_DLM}
\end{figure}
%
%----------------------------------
\paragraph{Boundary condition}
%-----------------------------------
%
With respect to Fig.~\ref{f:Enhanced_DLM}(a), the general form of the boundary condition (for an harmonic motion of the control point of the receiving panel, located at its 3/4 chord) is:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
i \omega \mathbf{h} e^{i\omega t} \cdot(\mathbf{n}_0 + \mathbf{r}e^{i\omega t} \times \mathbf{n}_0) = (\mathbf{u}_{\infty} + \mathbf{u}_{0} + \mathbf{u}_{1}e^{i\omega t}) \cdot (\mathbf{n}_0 + \mathbf{r}e^{i\omega t} \times \mathbf{n}_0)
\end{aligned}
\label{eq:boundary} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $\mathbf{h}$ and $\mathbf{r}$ are, respectively, the panel displacement and the rotation vectors for the considered motion at frequency $\omega$, $\mathbf{n}_0$ is the panel normal vector in its original position; $\mathbf{u}_{\infty}$ is the free stream velocity vector, $\mathbf{u}_{0}$ is the steady perturbation velocity vector due to trim and $\mathbf{u}_{1}$ is the unsteady perturbation velocity vector.
%
\par
%
Subtracting the steady boundary condition ($\mathbf{u}_{0} \cdot \mathbf{n}_0 = - \mathbf{u}_{\infty} \cdot \mathbf{n}_0$) and neglecting component $\mathbf{u}_{0} \cdot \mathbf{r}e^{i\omega t} \times \mathbf{n}_0$, Eq.~(\ref{eq:boundary}) leads to the general unsteady boundary condition:
%
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\mathbf{u}_{1} \cdot \mathbf{n}_0 = i \omega \mathbf{h} \cdot \mathbf{n}_0  - \mathbf{u}_{\infty} \cdot (\mathbf{r} \times \mathbf{n}_0)
\end{aligned}
\label{eq:boundary_perturb} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
With respect to the original DLM formulation, in which the aerodynamic model is not trimmed and $\mathbf{u}_{\infty}$ is always directed along the panel chord, in the current formulation the second term of the right hand side of Eq.~(\ref{eq:boundary_perturb}) features an extra contribution proportional to the angle of the attack of the wing and which takes into account yaw/dihedral coupling.
%
%
%----------------------------------
\paragraph{Forces}
%-----------------------------------
%
In the traditional formulation of the DLM, the downwash equation relates the pressure difference at the panel control point  with the normal to the panel component of the induced velocity. Pressure difference is due to the strength of an acceleration potential line located at the panel quarter chord.
%
\par
%
For the evaluation of the extra coupling contributions it is convenient to visualize the forces acting on the panel using the Kutta law. For an harmonic motion (see Fig.~\ref{f:Enhanced_DLM}(b) ) it is:
%
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\mathbf{F} = \rho \; \mathbf{V} \times \mathbf{\Gamma}
\end{aligned}
\label{eq:Kutta} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%
where $\mathbf{F}$ is the aerodynamic force on the panel load point, $\rho$ is the flow density and $\mathbf{V}$ is the total panel relative velocity, given by:
%
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\mathbf{V} = \mathbf{u}_{\infty} + \mathbf{u}_{0} + \mathbf{u}_{1}e^{i\omega t} - i \omega \mathbf{h} e^{i\omega t} 
\end{aligned}
\label{eq:panel_relative_velocity} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where vector $\mathbf{h}$ is now calculated at the one quarter chord load point and $\mathbf{\Gamma}$ is the unsteady bound vortex circulation vector, given by:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\mathbf{\Gamma} = \mathbf{\Gamma}_0 + \mathbf{\Gamma}_1  e^{i\omega t}  + \mathbf{r} e^{i\omega t} \times \mathbf{\Gamma}_0
\end{aligned}
\label{eq:Circulation} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%
In Eq.~(\ref{eq:Circulation}) $\mathbf{\Gamma}_0$ is the steady circulation due to trim and the second term is the unsteady contribution due to the change of intensity of the bound vortex while the third contribution is  due to the modal rotation of the steady circulation bound vortex. Developing Eq.~(\ref{eq:Kutta}) and removing the steady contribution to the force ($\mathbf{F}_0 = (\mathbf{u}_{\infty} + \mathbf{u}_0)\times \mathbf{\Gamma}_0$), the \textit{first harmonic} of the unsteady total force is given by:
%
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\mathbf{F}_1 =  (\mathbf{u}_{\infty} + \mathbf{u}_0)\times \mathbf{\Gamma}_1 \times (\mathbf{u}_{\infty} + \mathbf{u}_0)\times (\mathbf{r} \times \mathbf{\Gamma}_0) + (\mathbf{u}_{1} - \omega \mathbf{h}) \times  \mathbf{\Gamma}_0
\end{aligned}
\label{eq:Kutta_unsteady} 
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Where contributions of $\mathbf{u}_0$ are usually neglected as small compared to $\mathbf{u}_{\infty}$. The normal to the panel component of the first term of Eq.~(\ref{eq:Kutta_unsteady}) includes the only unsteady force component calculated by the traditional DLM and is due to unsteady circulation. It is worth mentioning that common implementations of the traditional DLM, as the one used within the context of this work, feature a Vortex Lattice Method (VLM) to evaluate the zero-frequency contribution of such term~\cite{Rodden_1968}. Contributions at non-zero frequencies use the downwash/pressure difference relation based on the acceleration potential theory. 
%
\par
%
The here presented enhanced DLM formulation features (for the zero-frequency unsteady force) a correct implementation of the first term of Eq.~(\ref{eq:Kutta_unsteady}), taking into consideration also in-plane forces and the corrected normal to the panel component, proportional to the angle of attack of the wing due to trim. 
%
\par
%
The correct evaluation of the trim condition by means of the embedded VLM method (i.e. the calculation of the correct $\mathbf{u}_{\infty}$ and $\mathbf{\Gamma}_0$ distribution for assigned asymptotic speed and mass of the model) also allows for the account of the third component of the unsteady force in Eq.~(\ref{eq:Kutta_unsteady}), responsible for yaw-roll coupling.  
%
\par
%
The second term of Eq.~(\ref{eq:Kutta_unsteady}) has not been included as it has been shown that its integration in the Generalized Force calculation procedure, in isolation from the quadratic mode shape components~\cite{VanZyl-2012,VanZyl-2012b,Segalman-1996}, may lead to wrong results.
%
%----------------------------------
\paragraph{Generalized Aerodynamic Forces}
%-----------------------------------
%
%Aerodynamic forces are evaluated by a DLM~\cite{Rodden_1968,Rodden_Taylor_1998}. 
The generalized aerodynamic forces  $\tilde{\mathbf{Q}}$ 
%$\tilde{\mathcalbf{Q}}$ 
acting on a thin lifting system are given for a harmonic oscillation of the structure at a certain reduced frequency $k$:
%
%---  EQ  ------------------------
\begin{equation}
\begin{aligned}
%\widetilde{\boldsymbol{f}}
%\inblue{\widetilde{\mathcalbf{Q}}} = q_\infty \widetilde{\bA}\left({ik}\right)  \boldsymbol{\eta}
\widetilde{\bf{Q}} = q_\infty \widetilde{\bA}\left({ik}\right)  \widetilde{\boldsymbol{\eta}}
\end{aligned}
\label{eq:RFA}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $\widetilde{\boldsymbol{\eta}}$ is the modal coordinate vector, which includes both rigid ($\widetilde{\boldsymbol{\eta}}_R$) and elastic ($\widetilde{\boldsymbol{\eta}}_E$) modes, $q_\infty$ is the dynamic pressure and $\widetilde{\bA}\left({ik}\right)$ is the Generalized Aerodynamic Force (GAF) matrix. 
The tilde is here used to specify that these generalized forces are relative to the generalized coordinates of the normal modes-based decomposition performed with respect to a reference system which is, in general, different than the stability axes used in Eqs.~(\ref{eq:lagrange_translation3}) to (\ref{eq:eom_deformation}). A transformation is needed to make them consistent with the primary Lagrangian coordinates $\bq$, as it will be discussed in section~\ref{sss:transf1}.
%
The  reduced frequency $k$ is obtained by normalizing the circular frequency $\omega$ with the free-stream velocity $V_\infty$ and the reference length $\hat{c}$, i.e., $k=\frac{\omega \, V_\infty }{ \hat{c} }$).
%
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Rational Function approximation} \label{sss:rational}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
The linear unsteady aerodynamic operator is of the transcendental kind in the Laplace domain, due to time delays in the propagation of disturbances (compressibility effects) and the convected wake vorticity~\cite{Gennaretti_MastroddiJoA2004}.
To overcome this difficulty, the operator is approximated by rational expressions involving a finite number of poles; in the time domain, thus, the aerodynamic forces are described by a finite number of states.
Typically, it holds:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\widetilde{\bA} (i k)  = \widetilde{\bA}_0  +
ik \, \widetilde{\bA}_1 +\left(i k  \right)^2 \widetilde{\bA}_2  +\text{High order terms}
\end{aligned}
\label{eq:RFA2}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
The part without higher-order terms represents a \emph{quasi-steady} approximation. Popular procedures to determine the higher-order terms in Eq.~(\ref{eq:RFA2}) are the so-called Rational Function Approximation (RFA) \cite{Roger1977,Karpel1982}, or alternatively, Rational Matrix Approximation (RMA) \cite{Morino_Mantegazza_1995AIAAJ}.
%
The approach considered in this paper is based on Roger's work~\cite{Roger1977}, and provides:
%The aerodynamic added states are expressed as \inred{[Ma questi non sono mica gli added states]}: 
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\widetilde{\bA} (i k)  = \widetilde{\bA}_0  +
ik \, \widetilde{\bA}_1 +\left(i k  \right)^2 \widetilde{\bA}_2  + \sum_{j=1}^{N_{\text{lag}}} \frac{ik}{ik+ \frac{\beta_j \hat{c}}{V_\infty}  } \widetilde{\bA}_{2+j}
\label{eq:Roger}
\end{aligned}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where $\beta_i$ are called lag coefficients and are set by the user.
%
\par 
%
The DLM calculates $\widetilde{\bA}$ for a selected set of reduced frequencies $k$ (and for a certain Mach number). 
To fit the provided data and  express $\widetilde{\bA}$ as shown in Eq.~(\ref{eq:Roger}), a least-square approach is pursued.  
Typically, the steady values $\widetilde{\bA}(0)$  determine  $\widetilde{\bA}_0$, and the fitting procedure involves matrices  $\widetilde{\bA}_j$ with $j>0$. 
%
\par 
%
It is important to notice that the fitting procedure can be fine-tuned to approximate better some regions of frequencies. 
To increase precision in the $k\rightarrow0$ region a modified Roger
%, addressed to as Roger Mod, i
is here implemented which adds to the original set of Least-Square constraints
%
%of Roger RFA over the values of $\widetilde{\bA} (i k)$ 
a further condition on the \emph{derivative} of the interpolated GAF matrix, as better explained in~\cite{UC3Mteam_PrP1ceas}.
%
%Such target derivative matrix is determined at $k=0$ on the basis of a finite difference scheme of the given $\widetilde{\bA} (i k)$. 
This method has proven to be useful to increase accuracy around the $k \rightarrow 0$ region of frequencies, where most of the flight dynamic physics is held, preserving, at the same time, good interpolation for higher frequencies characteristic of the aeroelastic behaviour. %~\cite{UC3Mteam_PrP1ceas}. 
%
%see also reference~\cite{UC3Mteam_PrP1ceas}) approach is used  in which the least square is performed imposing also the value of the derivative $\left. \frac{\ddi \widetilde{\bA}}{\ddi \,  ik} \right|_{k=0}$, obtained by numerical differentiation,  in the fitting process.  
%
\par 
%
%For $k=0$ and 
%\inred{[Questo ultimo paragrafo serve a qualcosa in concreto?]}
Neglecting higher-order terms, it holds that $\widetilde{\bA}_1 = \left. \frac{\ddi {\widetilde{\bA}}}{\ddi \,  ik} \right|_{k=0}$, and $\widetilde{\bA}_2 = \frac{1}{2} \left. \frac{\ddi^2 {\widetilde{\bA}}}{\ddi \,  (ik)^2} \right|_{k=0}$. 
%Matrices $\bA_1$ and $\bA_2$ can be evaluated with finite differences on DLM given $\bA(ik)$. 
Notice how this justifies the terminology \emph{quasi-steady}: the model is adequate in the region of small reduced frequencies. 
% physical lag phenomena are approximated about the steady condition not dominant.    
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Analytical continuation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
Invoking the \emph{analytical continuation}~\cite{Dettman_BOOK1969}, if an analytical function is known in terms of the imaginary variable $ik$, then, the same expression with $ik$ can be used for a the generic $p = g + ik$, and the function is finally described in the whole complex plane.
Thus, the above expressions can be extended just substituting $p$ (nondimensional Laplace variable) to $ik$.
%
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Rigid generalized coordinates and rigid modes}
\label{sss:transf1}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
In order to be consistent with Eq.~\ref{eq:lagrange}, 
%express the whole problem in terms of the a unique set of generalized coordinates
the modal rigid-body coordinates used in the DLM, Eq.~(\ref{eq:RFA}), need to be expressed in terms of rigid Lagrangian coordinates, Eq.~(\ref{eq:generalized_coordinate}). 
%
%The elastic part $\boldsymbol{\eta}_E$ does not have such an issue. % as they are in both  same generalized coordinates are used in both the DLM and the overall problem formulation. 
%
%\emph{rigid}
%Considering the rigid part only, there is the need to express the aerodynamic forces as function 
%Next step is to express the modal rigid-body coordinates (and derivatives) in terms of rigid generalized (Lagrangian) coordinates (and derivatives). This is needed as we would like to recast the whole problem using a unique set of ``rigid'' coordinates.
%
Such transformation depends on the reference flight condition; for the chosen one  (straight-and-level flight in stability- axes) and for the the longitudinal plane dynamics, it holds: 
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\widetilde{\boldsymbol{\eta}}_R =
\left\{{\begin{array}{c}
	\widetilde{\eta}_{R_x}\\
	\widetilde{\eta}_{R_z}\\
	\widetilde{\eta}_{R_{\theta_y}}\\
	\end{array}}\right\} = \underbrace{\left[\begin{array}{ccc}
\cos(\pi - AoA_{}) & \sin(\pi - AoA_{}) & 0  \\
-\sin(\pi - AoA_{}) & \cos(\pi - AoA_{}) & 0  \\
0 & 0 & 1 \\
\end{array}\right]}_{\bT_1}
\left\{{\begin{array}{c}
	x_E\\
	z_E\\
	\theta\\
	\end{array}}\right\}  
%= \bT^L_1  \left\{{\begin{array}{c}
%	x_E\\
%	z_E\\
%	\theta\\
%	\end{array}}\right\}
\end{aligned}
\label{eq:rmodes2rigidvector1_long}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%\boldsymbol{\eta_R} =
%\left\{{\begin{array}{c}
%   \eta_{T_y}\\
%   \eta_{R_x}\\
%   \eta_{R_z}\\
%\end{array}}\right\} = \left[\begin{array}{ccc}
%1 & 0 & 0  \\
%0 & -1 & 0  \\
%0 & 0 & -1 \\
%\end{array}\right]
% \left\{{\begin{array}{c}
%   y_E\\
%   \phi\\
%   \psi\\
%\end{array}}\right\}  = \bT_1  \left\{{\begin{array}{c}
%   y_E\\
%   \phi\\
%   \psi\\
%\end{array}}\right\}
%\end{aligned}
%\label{eq:rmodes2rigidvector1_lateral}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
%\left\{{\dot{\eta}^L_R}\right\} 
\boldsymbol{\dot{\widetilde{\eta}}}_R =
\left\{{\begin{array}{c}
   \dot{\widetilde{\eta}}_{R_x}\\
   \dot{\widetilde{\eta}}_{R_z}\\
   \dot{\widetilde{\eta}}_{R_{\theta_y}}\\
\end{array}}\right\} =& 
\underbrace{\left[\begin{array}{ccc}
0 & 0 & 0  \\
0 & 0 & V_\infty  \\
0 & 0 & 0 \\
\end{array}\right]}_{\bT_2} 
 \left\{{\begin{array}{c}
   x_E\\
   z_E\\
   \theta\\
\end{array}}\right\}+
 % \underbrace{\left[\begin{array}{ccc}
%\cos(\pi - AoA_{DLM}) & \sin(\pi - AoA_{DLM}) & 0  \\
%-\sin(\pi - AoA_{DLM}) & \cos(\pi - AoA_{DLM}) & 0  \\
%0 & 0 & 1 \\
%\end{array}\right]}_{\bT_3}%
\bT_3
 \left\{{\begin{array}{c}
   u\\
   w\\
   q\\
\end{array}}\right\}
%\\
%=& \bT^L_2  \left\{{\begin{array}{c}
%   x_E\\
%	z_E\\
%	\theta\\
%\end{array}}\right\}+
%\bT^L_3  \left\{{\begin{array}{c}
%    u\\
%	w\\
%	q\\
%\end{array}}\right\}
\end{aligned}
\label{eq:rmodes2rigidvector2_long}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%%\left\{{\dot{\eta}_R}\right\} 
%\boldsymbol{\dot{\eta}_R} =
%\left\{{\begin{array}{c}
%   \dot{\eta}_{T_y}\\
%   \dot{\eta}_{R_x}\\
%   \dot{\eta}_{R_z}\\
%\end{array}}\right\} =& \left[\begin{array}{ccc}
%0 & 0 & V_\infty  \\
%0 & 0 & 0  \\
%0 & 0 & 0 \\
%\end{array}\right]
% \left\{{\begin{array}{c}
%   y_E\\
%   \phi\\
%   \psi\\
%\end{array}}\right\}+
%  \left[\begin{array}{ccc}
%1 & 0 & 0  \\
%0 & -1 & 0  \\
%0 & 0 & -1 \\
%\end{array}\right]
% \left\{{\begin{array}{c}
%   v\\
%   p\\
%   r\\
%\end{array}}\right\}
%\\
%=& \bT_2  \left\{{\begin{array}{c}
%   y_E\\
%   \phi\\
%   \psi\\
%\end{array}}\right\}+
%\bT_3  \left\{{\begin{array}{c}
%   v\\
%   p\\
%   r\\
%\end{array}}\right\}
%\end{aligned}
%\label{eq:rmodes2rigidvector2_lateral}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
%\left\{{\ddot{\eta}_R}\right\} =
\boldsymbol{\ddot{\widetilde{\eta}}}_{R} =
\left\{{\begin{array}{c}
	\ddot{\widetilde{\eta}}_{R_x}\\
	\ddot{\widetilde{\eta}}_{R_z}\\
	\ddot{\widetilde{\eta}}_{R_{\theta_y}}\\
	\end{array}}\right\} =& \underbrace{\left[\begin{array}{ccc}
0 & 0 & 0  \\
0 & 0 & V_\infty  \\
0 & 0 & 0 \\
\end{array}\right]}_{\bT_4}
\left\{{\begin{array}{c}
	\dot{x}_E\\
	\dot{z}_E\\
	\dot{\theta}\\
	\end{array}}\right\}+
%\underbrace{\left[\begin{array}{ccc}
%\cos(\pi - AoA_{DLM}) & \sin(\pi - AoA_{DLM}) & 0  \\
%-\sin(\pi - AoA_{DLM}) & \cos(\pi - AoA_{DLM}) & 0  \\
%0 & 0 & 1 \\
%\end{array}\right]}_{\bT_5}
\bT_5
\left\{{\begin{array}{c}
	\dot{u}\\
	\dot{w}\\
	\dot{q}\\
	\end{array}}\right\}
%\\
%=& \bT^L_4  \left\{{\begin{array}{c}
%	\dot{x}_E\\
%	\dot{z}_E\\
%	\dot{\theta}\\
%	\end{array}}\right\}+
%\bT^L_5  \left\{{\begin{array}{c}
%	\dot{u}\\
%	\dot{w}\\
%	\dot{q}\\
%	\end{array}}\right\}
\end{aligned}
\label{eq:rmodes2rigidvector3_long}
\end{equation}
%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%%\left\{{\ddot{\eta}_R}\right\} =
%\boldsymbol{\ddot{\eta}_{R}} =
%\left\{{\begin{array}{c}
%   \ddot{\eta}_{T_y}\\
%   \ddot{\eta}_{R_x}\\
%   \ddot{\eta}_{R_z}\\
%\end{array}}\right\} =& \left[\begin{array}{ccc}
%0 & 0 & V_\infty  \\
%0 & 0 & 0  \\
%0 & 0 & 0 \\
%\end{array}\right]
% \left\{{\begin{array}{c}
%   \dot{y}_E\\
%   \dot{\phi}\\
%   \dot{\psi}\\
%\end{array}}\right\}+
%  \left[\begin{array}{ccc}
%1 & 0 & 0  \\
%0 & -1 & 0  \\
%0 & 0 & -1 \\
%\end{array}\right]
% \left\{{\begin{array}{c}
%   \dot{v}\\
%   \dot{p}\\
%   \dot{r}\\
%\end{array}}\right\}
%\\
%=& \bT_4  \left\{{\begin{array}{c}
%   {\dot{y}_E}\\
%   {\dot{\phi}}\\
%   \dot{\psi}\\
%\end{array}}\right\}+
%\bT_5  \left\{{\begin{array}{c}
%   \dot{v}\\
%   \dot{p}\\
%   \dot{r}\\
%\end{array}}\right\}
%\end{aligned}
%\label{eq:rmodes2rigidvector3_lateral}
%\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%\inblue{where $\boldsymbol{{\eta}}^L_{R}$ refers to the rigid modes in the longitudinal plane, being $\eta_{R_x}$ and  $\eta_{R_z}$ the translational ones, and $\eta_{R_{\theta_y}}$ the rotational one.}
%
where $\bT_3 =\bT_5 = \bT_1$,  $\widetilde{\eta}_{R_x}$, $\widetilde{\eta}_{R_z}$ and $\widetilde{\eta}_{R_{\theta_y}}$ are the modal coordinates of the three rigid modes in the longitudinal plane, and $AoA$ is the trim angle of attack, in radiant, for given asymptotic speed and mass of the vehicle with respect to the DLM reference system. 
%\inred{$AoA_{DLM}$ non mi piace ma non possiamo usare ne $\alpha$ ne $\theta$ per eviatare confusione. Nd Rocco.}
It is worth underlying that in the DLM reference system, axis $x$ is directed along the unperturbed asymptotic speed and $z$ axis is directed upward. 
%along the inertial $y$ 
%and $z comes as the cross product of the two.
%\inblue{where $x_E, \, z_E, \, u, \,  w, \, q$ represent perturbation quantities of the Lagrange generalized rigid coordinates that describe longitudinal motion [carefull what about theta?];    $\eta_{T_x}$, $\eta_{T_z}$, $\eta_{R_y}$ are the translational and rotational rigid modes in the DLM frame}.
%
%where $y_E, \, v, \, p, \, r$ represent perturbation quantities of the Lagrange generalized rigid coordinates that describe lateral-directional motion;    $\eta_{T_y}$, $\eta_{R_x}$, $\eta_{R_z}$ are the translational and rotational rigid modes in the DLM frame.
%
\inblue{[E' proprio necessario dirlo?]} Recall that  Eqs.~(\ref{eq:rmodes2rigidvector1_long}) to (\ref{eq:rmodes2rigidvector3_long}) %\ref{eq:rmodes2rigidvector1_lateral} to \ref{eq:rmodes2rigidvector3_lateral} 
hold if the rigid-body modes are selected to be of unitary translation/rotation, otherwise a scaling factor needs to be applied to the matrices to recover consistency with the generalized coordinates of Eq.~(\ref{eq:generalized_coordinate}).
%
The reader is referred to paper~\cite{UC3M_UFFDScitech} for the expression relative to the lateral-directional dynamics.
%\par
%
%It is important to remark that, in order to satisfy the mean-axes hypothesis, the rigid-body modes need to be selected orthogonal to each other. \inred{RIVEDERE QUESTO STATEMENT}
%
%\par
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Expressing the GAFs in the stability axes}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
The generalized forces obtained with the DLM need to be projected to be consistent with the Lagrangian coordinates of Eq.~(\ref{eq:generalized_coordinate}). 
%in which the overall problem is formulated. 
% expressed in terms of the generalized coordinates of the problem.
%This involves only the rigid generalized coordinates, as the elastic ones are coincident between DLM and the problem. 
%The projection can be performed with a matrix $\mathcalbf{R}$. 
With reference to Eq.~(\ref{eq:lagrange}) it holds:
%------
% EQ LONG
%-----
\begin{equation}
{\bf{Q}} =  \frac{\pd  \mathcal{W}}{\pd \bq}^T = \left[ \frac{\pd  \mathcal{W}}{\pd \boldsymbol{\widetilde{\eta}} } \cdot \frac{\pd \boldsymbol{\widetilde{\eta}} } {\pd \bq} \right]^T = \frac{\pd \boldsymbol{\widetilde{\eta}} } {\pd \bq}^T \cdot \frac{\pd  \mathcal{W}}{\pd \boldsymbol{\widetilde{\eta}} }^T
=\mathcalbf{R}^T\widetilde{\bf{Q}}= q_\infty \underbrace{ \mathcalbf{R}^T \widetilde{\bA} \left({ik}\right)}_{\bA(ik)} \boldsymbol{\widetilde{\eta}}
%%   = q_\infty {\bA}\left({ik}\right)  \boldsymbol{\eta}^L
\label{eq:rotated_forces}
\end{equation}
%-----------
%%------
%% EQ
%%-----
%\begin{equation}
%\boldsymbol{f} = \bR^{LD} \widetilde{\boldsymbol{f}}= q_\infty \bR^{LD} \widetilde{\bA}\left({ik}\right)  \boldsymbol{\eta} = q_\infty {\bA}\left({ik}\right)  \boldsymbol{\eta}
%\label{eq:rotated_forces}
%\end{equation}
%%-----------
%
%where the GAF matrix $\widetilde{\bA}$ has then been expressed in the Lagrangian coordinates. 
%
For the longitudinal dynamics $\mathcalbf{R}$ is:  %, which only takes into account the lateral-directional motion:
%------
% EQ LONG
%-----
\begin{equation}
\mathcalbf{R} = \left[ \begin{array}{cc}
%\left[\begin{array}{ccc}
%\cos(\pi - AoA_{}) & \sin(\pi - AoA_{}) & 0  \\
%-\sin(\pi - AoA_{}) & \cos(\pi - AoA_{}) & 0  \\
%0 & 0 & 1 \\
%\end{array}\right] 
\bT_1
& \boldsymbol{0}^{3 \x n_E}  \\ 
% \left[0_{3 \x n_E}\right] \\
%\left[0_{n_E \x 3}\right] & \left[I_{n_E}\right]
\boldsymbol{0}^{n_E \x 3}  & \boldsymbol{I}^{n_E} 
\end{array}\right]
\label{eq:rotation_matrix_long}
\end{equation}
%
%
\par 
%
In the case of the quasi-steady approximation, applying the inverse Fourier transform, the GAFs can be expressed as: 
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
{\bf{Q}} =  q_\infty \left( {\bA}_0  \, \boldsymbol{\widetilde{\eta}}  + \frac{\hat{c}}{V_\infty }{\bA}_1  \, \boldsymbol{\dot{\widetilde{\eta}}}  +  \frac{\hat{c}^2}{V_\infty^2}  {\bA}_2 \, \boldsymbol{\ddot{\widetilde{\eta}}}   \right)
\label{eq:faero_FT}
\end{equation}
%--------------------------------
%
%%------
%% EQ LAT
%%-----
%\begin{equation}
%\bR^{LD} = \left[ \begin{array}{cc}
%\left[\begin{array}{ccc}
%1 & 0 & 0 \\
%0 & -1 & 0 \\
%0 & 0 & -1 \\
%\end{array}\right] & \boldsymbol{0}_{3 \x n_E}  \\ % \left[0_{3 \x n_E}\right] \\
%%\left[0_{n_E \x 3}\right] & \left[I_{n_E}\right]
%\boldsymbol{0}_{n_E \x 3}  & \boldsymbol{I}_{n_E} 
%\end{array}\right]
%\label{eq:rotation_matrix_lateral}
%\end{equation}
%----------------
%
%where $n_E$ is the number of generalized coordinates relative to the elastic deformations.
%$\bR^{L}$  %$\bR^{LD}$ 
%needs to be applied to the DLM GAF matrix.  
%


==> chapters/IIc_Theory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    %
\subsection{State-Space Formulation} %
%                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%As discussed in the \inblue{section}~\ref{sss:perturb1}, for the chosen reference condition the linearized set of equations can be decoupled between longitudinal and lateral-directional dynamics~\cite{Etkin_2012}. 
In this section both sets of equations governing the dynamics of the rigid and flexible aircraft are considered. 
Considering that the coupling between rigid and elastic dynamics is introduced by the aerodynamic forces only, to model the dynamics of the flexible aircraft it is formally sufficient to augment system of Eqs.~(\ref{eq:lagrange_translation3}) and (\ref{eq:eqom_rotation_vectorial}) with Eq.~(\ref{eq:eom_deformation}) and extend the set of Lagrangian coordinates. 
%
\inblue{[Toglierei la frase seguente]}
Finally, the partitioning of aerodynamic forces will be addressed in \inblue{section}~\ref{sss:flexible_aerodynamics}.
%Being coupling between rigid and elastic dynamics introduced by aerodynamic forces only, it is possible to pass from the system relative to the rigid/flexible aircraft just considering the appropriate generalized coordinates and equations (only rigid, or rigid and elastic).
Only specialization for the longitudinal case is shown, reader is referred to~\cite{UC3M_UFFDScitech} for the expression relative to the lateral-directional dynamics.
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Rigid part of the aircraft dynamics}
\label{sss:rigidpart}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%\subsubsection{Rigid part of the Lateral-directional system}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%
The set of perturbation equations in state-space form governing the rigid part of the aircraft dynamics in stability axes~\cite{Etkin_2012} is:
%and specialized for the chosen reference condition is: 
% \inred{[necessario inserire parte che spiega la linerizzazione, check simboli tipo W0]}:
%
%---------------------------------
% EQ     LONG             |
%---------------------------------
\begin{equation}
\begin{aligned}
& \left[\begin{array}{cccccc}
m & 0 & 0 & 0 & 0 & 0 \\
0 & m & 0 & 0 & 0 & 0 \\
0 & 0 & I_{yy} & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 & 0 \\
0 & 0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 0 & 1 \\
\end{array}
\right] \left\{{\begin{array}{c}
	\dot{u}\\
	\dot{w}\\
	\dot{q}\\
	\dot{x}_E\\
	\dot{z}_E\\
	\dot{\theta}\\
	\end{array}}\right\} =
%& \left[\begin{array}{cccccc}
%0 & -mQ_0 & -mW_0 & 0 & 0 & -mg \cos{\Theta_0} \\
%mQ_0 & 0 & mU_0 & 0 & 0 & -mg \sin{\Theta_0} \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%\cos{\Theta_0} & \sin{\Theta_0} & 0 & 0 & 0 & -U_0\sin{\Theta_0}+W_0\cos{\Theta_0} \\
%-\sin{\Theta_0} & \cos{\Theta_0} & 0 & 0 &  0 & -(U_0\cos{\Theta_0}+W_0\sin{\Theta_0}) \\
%0 & 0 & 1 & 0 & 0 & 0 \\
%\end{array}
%\right]
& \left[\begin{array}{cccccc}
0 &  0 &   & 0 & 0 & -mg   \\
0 & 0 & mU_0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
1 & 0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 &  0 & -U_0 \\
0 & 0 & 1 & 0 & 0 & 0 \\
\end{array}
\right]
\left\{{\begin{array}{c}
	u\\
	w\\
	q\\
	x_E\\
	z_E\\
	\theta\\
	\end{array}}\right\}+\left\{{\begin{array}{c}
	{Q}_x \\
	{Q}_z \\
	{Q}_{\theta_y} \\
	0 \\
	0 \\
	0 \\
	\end{array}}\right\}
\end{aligned}
\label{eq:salf_matrix_long2}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%& \left[\begin{array}{cccccc}
%m & 0 & 0 & 0 & 0 & 0 \\
%0 & I_{xx} & -I_{xz} & 0 & 0 & 0 \\
%0 &-I_{xz} & I_{zz} & 0 & 0 & 0 \\
%0 & 0 & 0 & 1 & 0 & 0 \\
%0 & 0 & 0 & 0 & 1 & 0 \\
%0 & 0 & 0 & 0 & 0 & 1 \\
%\end{array}
%\right] \left\{{\begin{array}{c}
%   \dot{v}\\
%   \dot{p}\\
%   \dot{r}\\
%   \dot{y}_E\\
%   \dot{\phi}\\
%  \dot{\psi}\\
%\end{array}}\right\} =
%& \left[\begin{array}{cccccc}
%0 & 0 & -m \, V_{\infty} & 0 & mg & 0 \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 & 0 & 0 \\
%1 & 0 & 0 & 0 & 0 & V_{\infty} \\
%0 & 1 & 0 & 0 &  0 &0 \\
%0 & 0 & 1 & 0 & 0 & 0 \\
%\end{array}
%\right]
%\left\{{\begin{array}{c}
%   v\\
%   p\\
%   r\\
%   y_E\\
%   \phi\\
%  \psi\\
%\end{array}}\right\}+\left\{{\begin{array}{c}
%   f_{R_y} \\
%   m_{R_x} \\
%   m_{R_z} \\
%   0 \\
%   0 \\
%   0 \\
%   \end{array}}\right\}
%\end{aligned}
%\label{eq:salf_matrix_lateral2}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
being the considered rigid state:
%
%---------------------------------
% EQ    LONG              |
%---------------------------------
\begin{equation}
\begin{aligned}
\bx_R = \left\{{\begin{array}{c}
	u\\
	w\\
	q\\
	x_E\\
	z_E\\
	\theta\\
	\end{array}}\right\} 
\hspace{.8cm}
\begin{array}{c}
\rightarrow longitudinal~velocity   \\ 
\rightarrow vertical~velocity~(\sim \alpha V_\infty)  \\ 
\rightarrow pitch~rate \\
\rightarrow longitudinal~position \\
\rightarrow vertical~position \\
\rightarrow 2nd~Euler~angle
\\
\end{array}
\end{aligned}
\label{eq:rigid_state_salf_long}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%---------------------------------
%% EQ                  |
%%---------------------------------
%\begin{equation}
%\begin{aligned}
%\bx_R^{LD} = \left\{{\begin{array}{c}
%   v\\
%   p\\
%   r\\
%   y_E\\
%   \phi\\
%  \psi\\
%\end{array}}\right\}
% \hspace{.8cm}
%  \begin{array}{l}
%                \rightarrow lateral~velocity   \\
%                \rightarrow roll~velocity  \\
%           	\rightarrow yaw~velocity \\
%           	\rightarrow lateral~position \\
%           	\rightarrow 1st~Euler~angle \\
%           	\rightarrow 3rd~Euler~angle
%           	\\
%             \end{array}
%             \end{aligned}
%\label{eq:rigid_state_salf_lateral}
%\end{equation}
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%Recall, once again, that a rigid or flexible aircraft will lead to generally different values of such forces. 
%
%The above state vector will be indicated with $\bx_R^{L}$. 
%As it will be shown in the next sections, modeling the aerodynamics with higher-order terms will lead to an augmented state-vector. Moreover, in the case of flexible aircraft, the overall state vector will also include the generalized coordinates relative to the elastic part.
%
\par
The above system of Eq.~(\ref{eq:salf_matrix_long2}) can be condensed as:
%The rigid part of the generalized coordinates will be indicated with $\bx_R^{LD}$, and the above system can be condensed as:
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bM_{RR} \;  \dot{\bx}_R = \bK_{RR} \; \bx_R + \mathbf{Q}_{R}
\end{aligned}
\label{eq:rigid_matrix_salf2_long}
%\begin{aligned}
%\bM_{RR}^{LD} \;  \dot{\bx}_R^{LD} = {\bK_{RR}^{LD}} \; {\bx_R^{LD}} + \boldsymbol{f}_{R}^{LD}
%\end{aligned}
%\label{eq:rigid_matrix_salf2_lateral}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
where and $\mathbf{Q}_R = \left({Q}_x, {Q}_z, {Q}_{\theta_y} \right)^T$ are the GAF components relative to the longitudinal rigid motion. 
%longitudinal part of the generalized coordinates. 
%\inblue{In the following of the paper the superscript $L$ is dropped: each equation can be specialized for the longitudinal or lateral-directional cases considering the appropriate matrices/vectors}. % as only the lateral-directional dynamics is considered. 
%
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Rigid aircraft with quasi-steady aerodynamics}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%
With respect to system of Eq.~(\ref{eq:rigid_matrix_salf2_long}), let's consider the quasi-steady form of the GAF expressed in terms of generalized coordinates of Eq.~(\ref{eq:faero_FT}). 
Being only the rigid modes involved, the GAF matrices $\bA_i$ are indicated with $\bA_{i_{RR}}$. 
%
The aerodynamic force vector becomes then:
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
{\mathbf{Q}}_R =  q_\infty \left( \bA_{0_{RR}}  \, \boldsymbol{\widetilde{\eta}}_R  + \frac{\hat{c}}{V_\infty } \bA_{1_{RR}} \, \boldsymbol{\dot{\widetilde{\eta}}}_R  +  \frac{\hat{c}^2}{V_\infty^2}  \bA_{2_{RR}} \, \boldsymbol{\ddot{\widetilde{\eta}}}_R   \right)
\end{equation}
%--------------------------------
%  
%\inblue{in which the contribution to the perturbation equation of the aerodynamic forces acting in the reference condition has been temporarily omitted.} \inred{Non capisco. Nd Rocco}
%
Transforming the modal rigid-body coordinates ( Eqs.~(\ref{eq:rmodes2rigidvector1_long}), (\ref{eq:rmodes2rigidvector2_long}) and (\ref{eq:rmodes2rigidvector3_long}) ) and recalling the expression of the state vector of Eq.~(\ref{eq:rigid_state_salf_long}) it is possible to obtain an expression suitable for the state-space form:
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{multline}
\label{eq:rigidquasisteady}
{\mathbf{Q}}_R =  q_\infty \left( \left[ 
\begin{array}{cc}
\boldsymbol{0}^{n_R \times 1}  &  \bA_{0_{RR}} \bT_1 
\end{array}
\right] +   
\frac{\hat{c}}{V_\infty}   \left[ 
\begin{array}{cc}
\bA_{1_{RR}} \bT_3  &   \bA_{1_{RR}} \bT_2 
\end{array}
 \right]   
% \, \boldsymbol{\eta_R}  + \frac{b}{V_\infty } \bA_{1_{RR}} \, \boldsymbol{\dot{\eta}_R}  +  \frac{b^2}{V_\infty^2}  \bA_{2_{RR}} \, \boldsymbol{\ddot{\eta}_R}   
\right)  \bx_R^{}  + \\
q_\infty \left(   
\frac{\hat{c}^2}{V^2_\infty}   \left[ 
\begin{array}{cc}
\bA_{2_{RR}} \bT_5  &   \bA_{2_{RR}} \bT_4 
\end{array}
\right]   
% \, \boldsymbol{\eta_R}  + \frac{b}{V_\infty } \bA_{1_{RR}} \, \boldsymbol{\dot{\eta}_R}  +  \frac{b^2}{V_\infty^2}  \bA_{2_{RR}} \, \boldsymbol{\ddot{\eta}_R}   
\right)  \dot{\bx}_R^{}
\end{multline}
%--------------------------------
%    
The state-space system is then completely defined, and stability analysis can be trivially performed. 
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ {eq:rotation_matrix_long} {eq:rigidquasisteady}
\subsubsection{Interpretation of DLM-based GAFs with aerodynamic derivatives}
\label{sss:aerod_derivatives}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%\inblue{Generally, DLM forces need to be corrected for several main reasons. First, due to  flow assumptions, the DLM is not capable of describing  aerodynamic nonlinearities. The reader is referred to \cite{UC3M_NITRO,altri} for possible ways of correcting  for these deficiencies. %
%Even for flow behaving in an almost "ideally", 
%Secondly, due to its inherent formulation, the DLM is not able to evaluate forces along the airflow direction. This has relevant consequences for the evaluation of some aerodynamic derivatives regulating both the longitudinal and lateral-directional response. For this reason, the correction proposed in \cite{Kier_2009} has been implemented in the in-house DLM. Briefly, for the steady part of DLM kernel, evaluated by means of a Vortex Lattice Method (VLM), the Kutta-Joukowski formula $\rho \bV \x \boldsymbol{\Gamma}$ is used considering the actual acting velocity on the bound vortex (load point), instead  of the undisturbed flow one.}
It is possible to provide interpretation to most of the GAF entries in the case of quasi-steady aerodynamic modeling. 
The easiest case is the one with $AoA=0$: 
%of no trimmed aircraft for the evaluation of the DLM-based GAFs ($AoA=0$): 
in this case, in fact, the reader will notice that the rotation matrices in Eqs.~(\ref{eq:rotated_forces}) and (\ref{eq:rigidquasisteady}) are trivial, being the DLM reference system and the stability axes simply rotated along the common y axis of 180$^\circ$.
%
\par
%
%
%\inblue{As byproduct of the linearization of equations of motion, aerodynamic forces in the reference condition enter the forces on the right hand side of Eq.~(\ref{eq:salf_matrix_long2}).}
%
With reference to formulations proposed in \cite{Etkin_2012,Schmidt2012} for the longitudinal perturbation dynamics, the aerodynamic forces can be expressed as:
	% \ref{sss:rigidpart}  , do section~\ref{sss:transf1} lso correction are needed to augment the information the DLM is not able to}
\begin{equation}
\begin{aligned}
\left\{{\begin{array}{c}
	\mathcal{Q}_x \\
	\mathcal{Q}_z \\
	\mathcal{Q}_{\theta_y} \\
	0 \\
	0 \\
	0 \\
	\end{array}}\right\} = & q_\infty
\left[\begin{array}{cccccc}
-\frac{S}{V_\infty}(2C_{D_0}+C_{D_u}) & -\frac{S}{V_\infty}(C_{D_\alpha}-C_{L_0}) & -\frac{Sc}{2V_\infty}(C_{D_q}+C_{D_{\dot{\alpha}}}) & 0 & 0 & 0 \\
-\frac{S}{V_\infty}(2C_{L_0}-C_{L_u}) & -\frac{S}{V_\infty}(C_{L_\alpha}+C_{D_0}) & -\frac{Sc}{2V_\infty}(C_{L_q}+C_{L_{\dot{\alpha}}}) & 0 & 0 & 0 \\
\frac{Sc}{V_\infty}(2C_{m_0}+C_{m_u})&  \frac{Sc}{V_\infty}C_{m_\alpha} & \frac{Sc^2}{2V_\infty}(C_{m_q}+C_{m_{\dot{\alpha}}}) & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
\end{array} \right]
\left\{{\begin{array}{c}
	u\\
	w\\
	q\\
	x_E\\
	z_E\\
	\theta\\
	\end{array}}\right\} + \\
& q_\infty \left[\begin{array}{cccccc}
0 & -\frac{Sc}{2V_\infty^2}C_{D_{\dot{\alpha}}} & 0 & 0 & 0 & \frac{Sc}{2V_\infty}C_{D_{\dot{\alpha}}} \\
0 & -\frac{Sc}{2V_\infty^2}C_{L_{\dot{\alpha}}} & 0 & 0 & 0 & \frac{Sc}{2V_\infty}C_{L_{\dot{\alpha}}} \\
0 &  \frac{Sc^2}{2V_\infty^2}C_{m_{\dot{\alpha}}} & 0 & 0 & 0 & -\frac{Sc^2}{2V_\infty}C_{m_{\dot{\alpha}}} \\
0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 \\
\end{array} \right]
\left\{{\begin{array}{c}
	\dot{u}\\
	\dot{w}\\
	\dot{q}\\
	\dot{x}_E\\
	\dot{z}_E\\
	\dot{\theta}\\
	\end{array}}\right\}
\end{aligned}
\label{eq:rigid_matrix_salf}
\end{equation}
%
where $c$ is the typical length used in the normalization of the aerodynamic coefficients. Typically, in the longitudinal plane $\hat{c} = c/2$. It is highlighted how derivatives with respect to $\dot{\alpha}$ have been added and subtracted in correspondence of the columns of of $q$ and $\dot{\theta}$, taking advantage of the kinematic equation $\dot{\theta} = q$. This is because of the DLM method of force calculation, for which a pitch perturbation mode contains both a pitch rate ($q$) and a change of the asymptotic speed direction ($\dot{\alpha}$).
%
\par
%
Comparing Eq.~(\ref{eq:rigid_matrix_salf}) and  Eq.~(\ref{eq:rigidquasisteady}), for quasi-steady aerodynamics it holds that:  
%
\begin{equation}\label{eq:A0_coef}
\bA_{0_{RR}} = \left[\begin{array}{ccc}
0 & 0 & S(C_{D_\alpha}-C_{L_0}) \\
0 & 0 & S(C_{L_\alpha}+C_{D_0}) \\
0 & 0 & S c (C_{m_\alpha})
\end{array}\right]
\end{equation}
%
\begin{equation}\label{eq:A1_coef}
\bA_{1_{RR}} = \left[\begin{array}{ccc}
-2S(2C_{D_0}+C_{D_u}) & -2S(C_{D_\alpha}-C_{L_0}) & S(C_{D_q}+C_{D_{\dot{\alpha}}}) \\
-2S(2C_{L_0}+C_{L_u}) & -2S(C_{L_\alpha}+C_{D_0}) & S(C_{L_q}+C_{L_{\dot{\alpha}}}) \\
-2S(2C_{m_0}+C_{m_u}) & -2S(C_{m_\alpha}) &         S(C_{m_q}+C_{m_{\dot{\alpha}}}) \\
\end{array}\right]
\end{equation}
%
\begin{equation}\label{eq:A2_coef}
\bA_{2_{RR}} = \left[\begin{array}{ccc}
a_{11} & -S(C_{D_{\dot{\alpha}}}) & a_{13} \\
a_{21} & -S(C_{L_{\dot{\alpha}}}) & a_{23} \\
a_{31} & -S(C_{m_{\dot{\alpha}}}) & a_{33} \\
\end{array}\right]
\end{equation}
%
Notice that coefficients $C_{L_0}$ and $C_{D_0}$ cannot be directly computed by the enhanced-DLM. 
However, within the quasi-steady aerodynamics assumption, they can be evaluated by other means and integrated into the system. 
%to reflect the aerodynamic forces in the perturbation equations. 

%the matrices $\bA_{0_{RR}}$, $\bA_{1_{RR}}$ and $\bA_{2_{RR}}$ as obtained directly with the DLM cannot satisfy the above equivalences. With reference to  equation \ref{eq:A0_coef}, the DLM can predict only $C_{L_\alpha}$ and  $C_{m_\alpha}$, in the (3,2) and (3,3) entries.
%
%If ones accepts the quasi-steady aerodynamics approximation, the, is possible to have external evaluation of $C_{L_0}$ and $C_{D_0}$ to correct $\bA_{0_{RR}}$ matrix. Similar discussion holds for matrix $\bA_{1_{RR}}$ which also involves other aerodynamic coefficients as the ones relative to $C_D$, or with respect to $u$. 
%
When the same approach is repeated for the lateral-directional dynamics, the enhanced DLM can predict all terms (with the expected level of accuracy relative to the method). 
%, thus no further correction is needed to be performed
More on this aspect can be found in \cite{Baldelli_JoA2006,Auricchio_MS,Castellanos2019MScThesis}. 
%
\par
%
The authors remark that the interpretation of the GAF matrices in terms of aerodynamic derivative coefficients, as shown in Eq.~(\ref{eq:A1_coef}) and (\ref{eq:A2_coef}) does not hold anymore when added states are considered, as it can be trivially verified recalling Eq.~\ref{eq:Roger}. 
%
For the same reason, when higher-order terms are retained in the aerodynamic RFA (see Eq.~(\ref{eq:RFA2}) it becomes more cumbersome to integrate the coefficients $C_{L_0}$ and $C_{D_0}$ into the system. 
\inblue{An alternative approach, based on performing RFA before forming the GAF matrices could circumvent such issue, as explained in references~\cite{Kier2009UNIFYINGMA,Kier2011AnIL}.}
%
% As there is not an immediate correspondence at $k \rightarrow 0$ matrices$\bA_{1_{RR}}$ and $\bA_{2_{RR}}$} .
%
\par
%
%The intrinsic limitation in predicting accurately some of the aerodynamic derivatives by codes relying on potential method is well-known. However, the purpose of this paper is to show preliminary  effects of coupling between the flight-dynamics and aeroelasticity on an unconventional configuration of the Box Wing class rather than having a higher-fidelity quantitative estimation. 
%Hence, no corrections on the aerodynamic derivatives is performed. 
%
Finally, it is observed that most relevant flight-dynamic/aeroelastic interactions are not influenced by omission of such terms, hence, they are not considered in this study. 
%
%in the  longitudinal case the short-period, proven to be not strongly influenced by the coefficients not predicted by the DLM, results of this study will only be relative to the DLM-predicted aerodynamic forces not corrected. 
%
%
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsubsection{Flexible aircraft with quasi-steady aerodynamics}
\label{sss:flexible_aerodynamics}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
To take into account the dynamics of the flexible aircraft, Eq.~(\ref{eq:eom_deformation}) is added to the system of Eq.~(\ref{eq:rigid_matrix_salf2_long}) and the rigid state vector $\bx_R$  is augmented with the elastic coordinates $\boldsymbol{\eta}_{E}$, obtaining: 
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\begin{aligned}
\bx^{} = \left\{{\bx_R^{T}}; \dot{\boldsymbol{\eta}}_{E}^T ,  \boldsymbol{\eta}_{E}^T \right\}^T
\end{aligned}
\label{eq:rigid_matrix_salf3_lateral}
\end{equation}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
Consider now the quasi-steady form of the GAFs Eq.~(\ref{eq:faero_FT}). 
It is convenient to partition the matrices $\bA_i$ in terms of GAFs relative to rigid ($R$) and elastic ($E$) modes. It holds, then:
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\bA_i = \left[ \begin{array}{cc}
 \bA_{i_{RR}} &  \bA_{i_{RE}}  \\
 \bA_{i_{ER}} &  \bA_{i_{EE}}
\end{array}\right]
\label{eq:aero_coupling}
\end{equation}
%--------------------------------
%
Expressing the modal rigid-body coordinates in terms of rigid Lagrangian coordinates, Eqs.~(\ref{eq:rmodes2rigidvector1_long}), (\ref{eq:rmodes2rigidvector2_long}) and (\ref{eq:rmodes2rigidvector3_long}),  it is possible to refer the aerodynamic forces in terms of the state vector. %
%  
The problem can be recast in the following state-space form:
%
%
%---------------------------------
% EQ                  |
%---------------------------------
\begin{equation}
\resizebox{\hsize}{!}{$
\begin{aligned}
\left[\begin{array}{c|c|c}
\left({\bM_{RR}^{}}-q_\infty\left(\frac{\hat{c}}{V_\infty}\right)^2\left[{\begin{array}{cc}
   \bA_{2_{RR}} \bT_5 & \bA_{2_{RR}} \bT_4\\
   \boldsymbol{0}^{n_R} & \boldsymbol{0}^{n_R} \end{array}}
%\left[0_{n_R}\right] & \left[0_{n_R}\right]\end{array}}
   \right]\right) &
   \left[\begin{array}{c}
-q_\infty\left(\frac{\hat{c}}{V_\infty}\right)^2 \bA_{2_{RE}} \\
%\left[0_{n_R \x n_E}\right]  
\boldsymbol{0}^{n_R \x n_E} 
\end{array} \right] &
\boldsymbol{0}^{2n_R \x n_E}  \\ \\
%\left[ 0_{2n_R \x n_E}\right] \\ \\
\hline
-q_\infty\left(\frac{\hat{c}}{V_\infty}\right)^2 \bA_{2_{ER}} \left(\bT_5~~\bT_4 \right) &
\left( \mathbf{M_{EE}} -q_\infty\left(\frac{\hat{c}}{V_\infty}\right)^2 \bA_{2_{EE}}\right)&
\boldsymbol{0}^{n_E} \\ \\ \hline
%\left[ 0_{n_E}\right] \\ \\ \hline
%\left[0_{n_E \x 2n_R}\right] & \left[ 0_{n_E}\right] & \left[ I_{n_E}\right]
\boldsymbol{0}^{n_E \x 2n_R}  & \boldsymbol{0}^{n_E}  & \boldsymbol{I}^{n_E} %\left[ I_{n_E}\right]
\end{array} \right]
\left\{{\begin{array}{c}
   \dot{\bx}_R \\
   \ddot{\boldsymbol{\eta}}_E\\
   \dot{\boldsymbol{\eta}}_E\\
\end{array}}\right\}=
\\ \\
% right-hand side
\left[\begin{array}{c|c|c}
 \bK_{RR}^{} + q_\infty\left(

   \left[{\begin{array}{cc}
   \frac{\hat{c}}{V_\infty}\bA_{1_{RR}} \bT_3 & \frac{\hat{c}}{V_\infty}\bA_{1_{RR}} \bT_2 + \bA_{0_{RR}} \bT_1 \\
   \boldsymbol{0}^{n_R} & \boldsymbol{0}^{n_R} \end{array}}
   \right]
   \right) &  \left[\begin{array}{c}
\frac{q_\infty \hat{c}}{V_\infty}\bA_{1_{RE}} \\
\boldsymbol{0}^{n_R \x n_E }
\end{array} \right] & \left[\begin{array}{c}
q_\infty \bA_{0_{RE}} \\
\boldsymbol{0}^{n_R \x n_E }
\end{array} \right]\\ \\ \hline
q_\infty\left(
   \left[{\begin{array}{cc}
   \frac{\hat{c}}{V_\infty}\bA_{1_{ER}} \bT_3 & \frac{\hat{c}}{V_\infty}\bA_{1_{ER}} \bT_2 +\bA_{0_{ER}} \bT_1 \end{array}}
   \right]
   \right) &
   -\left( \mathbf{C_{EE}} -\frac{q_\infty \hat{c}}{V_\infty} \bA_{1_{EE}} \right) &
   -\left( \mathbf{K_{EE}} -q_\infty \bA_{0_{EE}} \right) \\ \\ \hline
   \boldsymbol{0}^{n_E \x 2n_R }  &  \boldsymbol{I}^{n_E}  & \boldsymbol{I}^{n_E}
\end{array} \right]
\left\{{\begin{array}{c}
   {\bx}_R \\
   \dot{\boldsymbol{\eta}}_E\\
   {\boldsymbol{\eta}}_E\\
\end{array}}\right\}
\end{aligned} $
}
\label{eq:matrix_nolag}
\end{equation} 
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%

The same approach can be used for the lateral-directional dynamics as detailed in efforts~\cite{UC3M_UFFDScitech,Castellanos2019MScThesis}.
%
\par
%
When unsteady aerodynamics is considered, the system is augmented with aerodynamic added states.  
The final state-space system  depends on the chosen model-lag augmentation technique (RFA/RMA), and, for the sake of brevity, is not shown here. The interested reader is referred to effort~\cite{Auricchio_MS} for more details.
%


==> chapters/VI_Conclusions.tex <==
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Application of a unified flight dynamic and aeroelastic in-house framework for the stability analysis of a free-flying PrandtlPlane configuration is shown. 
The investigation covers both longitudinal and lateral-directional planes and aims at assessing the mutual interaction between the two disciplines on the stability of the considered configuration. 
%
\par 
%
First, the formulation is shown and discussed. An enhanced DLM method is used for forces evaluation and a Roger-based Rational Function Approximation strategy is used to interpolate such forces over the range of frequencies of interest. Interpretation of steady and unsteady terms, by means of aerodynamic derivatives, is shown in case of quasi-steady approximation of the aerodynamic forces.
%
\par 
%
Coupled analyses are performed at cruise speed for two selected altitudes (i.e. sea and cruise levels).
First, the longitudinal plane is addressed. Flying qualities of the Short Period are assessed for both the rigid and the elastic configurations. A remarkable degradation in terms of damping ratio of the Short Period pole is noticed when considering the elastic configuration, as opposed to the rigid one. As for the aeroelastic behaviour of the Free-Flying configuration, the stability diagram shows a flutter free scenario for the considered speed range as opposed to the one of the Cantilever configuration. The raise in flutter speed has been interpreted as a synergistic effect of the interaction between the elastic and Short Period modes and the change in structural properties of the Free-Flying configuration with respect to the Cantilever one. 
%
\par 
%
Finally, lateral-directional plane is investigated. Flying qualities of the Dutch Roll are compared between the rigid and the elastic configurations. 
In this case, as well, taking into account the elasticity of the vehicle results in a degradation of the pole damping ratio. 
For this case, moreover, the effect of using an enhanced DLM method for aerodynamic forces calculation is investigated. 
Results show how Duch Roll poles shift towards the imaginary axis. This highlight how and more inclusive aerodynamic forces calculation method is crucial for a correct prediction of the lateral-directional dynamics.
Aeroelastic behaviour showed a considerably low flutter speed, which was proven not to be directly related to the aerodynamic rigid/elastic interaction. On the contrary, such an interaction shows to be slightly beneficial on the flutter onset.









%
\par 
%
%Then, the framework was applied to the rigid case aircraft, and classic flight dynamics was studied. 
%Integration of DLM aerodynamics, typically used for aeroelastic studies, allowed assessing the relevance of unsteady terms. 
%Within a quasi-steady approximation, 
%In particular, the derivative $C_{n \dot{\beta}}$  has been found to contribute to Dutch roll eigenvalue to a significant extent. 
%properties be
%the most significant ones. 
%\inred{Rodrigo is right now performing simulations excluding selectively $C_{Y_{dot{beta}}}$,  $C_{l_{dot{beta}}}$ and  $C_{n_{dot{beta}}}$ so we might tell which of the three is the most relevant}. 
%
%Dutch roll behavior of the rigid PrandtlPlane was then assessed with respect to the flying qualities requirements, showing to fall, according to MIL-F-878C, within the level 2 interval in cruise condition. 
%
%\par 
%
%Finally, the free-flying elastic case was considered. In terms of flight dynamics, the Dutch roll eigenvalue shifted considerably, and the flying qualities almost dropped to level 3, as a consequence of the rigid/elastic interaction. 
Aeroelastic behavior showed a considerably low flutter speed, which was proven not to be directly related to the aerodynamic rigid/elastic interaction.  On the contrary, such an interaction is proven to be slightly beneficial on the flutter onset.  
 
  

==> chapters/V_Results.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Several analyses are carried out on the testcase PrandtlPlane configuration. 
First, flying qualities are evaluated for the rigid aircraft, and effects of the unsteady aerodynamic terms is assessed. 
Then, the analysis of the flexible aircraft is carried out. 
Focus is on how flying qualities are affected by taking into account structural flexibility and at what extent flight dynamic affects the aeroelastic response. 
%
\par 
%
In this effort, the MTOW configuration is considered. Moreover, the aircraft is at straight-and-leveled flight. 
Flying qualities have been quantitatively assessed at sea level and nominal altitude cruise conditions, namely, $V_\infty=196~m/s$ at sea level, and  $V_\infty=252~m/s$ at an altitude of $10500~m$ (corresponding to a Mach number of 0.85).
%
\par
Given the comparative purpose of this investigation, even if flying at Mach number far from zero, the flow has been approximated as incompressible. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %
\subsection{Rigid flight dynamics}    %
%                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The aerodynamic derivatives as evaluated by AVL are given in Table~\ref{t:AVL_coeff}.   
%
%----------------------------
%     TABLE       |
%----------------------------
\begin{table}[!ht]
	\centering
	\begin{tabular}{lrlrlr}
		\toprule
		\multicolumn{2}{c}{Roll rate $p$} & \multicolumn{2}{c}{Yaw rate  $r$} & \multicolumn{2}{c}{Sideslip $\beta$ }\\ \midrule
		%$C_{L_p}$ &  0.000000 &  $ C_{L_r}$ &  -0.000000 & $C_{L_\beta}$ & -0.000000 \\
		$C_{Y_p}$ & -0.086515 &  $ C_{Y_r}$ &   0.207404 & $C_{Y_\beta}$ & -0.529050 \\
		$C_{l_p}$ & -0.502033 &  $ C_{l_r}$ &  -0.003751 & $C_{l_\beta}$ &  0.017207 \\
		%$C_{m_p}$ & -0.000000 &  $ C_{m_r}$ &  -0.000000 & $C_{m_\beta}$ & -0.000000 \\
		$C_{n_p}$ &  0.003417 &  $ C_{n_r}$ &  -0.071802 & $C_{n_\beta}$ &  0.030565 \\ \bottomrule
	\end{tabular}
	\caption{AVL rigid-body lateral stability derivatives.}
	\label{t:AVL_coeff}
\end{table}
%----------------------------
%
Results of stability analysis performed with \emph{Albatross} are shown in Figure~\ref{f:RL_ALBATROS}. 
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/RL_ALBATROS.pdf}
	\caption{Stability analysis for the rigid aircraft performed with \emph{Albatross} (only steady aerodynamics considered).}
	\label{f:RL_ALBATROS}
\end{figure}
%----------------------------|
%
In the two different cruise conditions, the eigenvalues relative to the Dutch roll mode are $-0.1298 \pm 0.5586 i$ (sea level) and $-0.08167 \pm 0.4102 i$ (nominal cruise altitude).  
According to flying-qualities regulations set by the MIL-F-878C for class III vehicles, Table~\ref{t:MILF}, the current aircraft fits in the level II category for flight phase B (which comprehends cruise). 
%
%----------------------------
%     TABLE                 |
%----------------------------
\begin{table}[!ht]
	\centering
	\begin{tabular}{|ccccc|}
		\hline
		FQ Level & \begin{tabular}[c]{@{}c@{}}Flight Phase\\ Category\end{tabular} & \multicolumn{1}{c}{Min $\zeta_{d}$} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Min $\zeta_{d} \omega_{nd}$\\ {[}rad/s{]}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Min $\omega_{nd}$\\ {[}rad/s{]}\end{tabular}} \\ \hline
		\multirow{3}{*}{1} & A & 0.19 & 0.35 & 0.4 \\
		& B & 0.08 & 0.15 & 0.4 \\
		& C & 0.08 & 0.10 & 0.4 \\ \hline
		2 & All & 0.02 & 0.05 & 0.4 \\ \hline
		3 & All & 0.00 & 0.00 & 0.4 \\ \hline
	\end{tabular}
	\caption{Flying-quality level requirements for Dutch roll according to the MIL-F-878C; aircraft of class III.}
	\label{t:MILF}
\end{table}
%----------------------------
%
%
%
\subsubsection{Effects of unsteady terms}
%
UFFD framework can be also used for the rigid aircraft by not including the elastic Lagrangian coordinates. % states in the formulation. 
As already underlined in the theoretical section, integration of the DLM aerodynamics enables to naturally include unsteady effects. 
It is then possible, with an ad-hoc procedure, to selectively assess the contribution of each unsteady terms to the flying qualities. 
According to  effort~\cite{UC3Mteam_PrP1ceas}, for the same configuration, the $C_{m_{\dot{\alpha}}}$ proved to change sensibly the short-period response. Hence, the interest in assessing analogous effects in the lateral-directional dynamics.
%
\par 
%
If one considers the quasi-steady approximation (i.e., no higher-order terms in equation \ref{eq:RFA2}), the GAF coefficients do retain a recognizable physical meaning~\cite{Baldelli_JoA2006}. Namely: 
%
%---------------------------------
% EQ                             |
%---------------------------------
\begin{equation}
 {\bA}_0 =\left[\begin{array}{ccc}
	0 & 0 &  S \, C_{Y_\beta}  \\
	0 & 0 & -S \, b \, C_{l_\beta}  \\
	0 & 0 & -S \, b \, C_{n_\beta}  \\
\end{array}\right]
\label{eq:A0_coeff}
\end{equation}
%---------------------------------
%
and
%
%---------------------------------
% EQ                             |
%---------------------------------
\begin{equation}
{\bA}_1 =\left[\begin{array}{ccc}
\frac{S}{\hat{c}} C_{Y_\beta}  & -\frac{Sb}{2\hat{c}} C_{Y_p}   &  -\frac{Sb}{2\hat{c}} \left( C_{Y_r} - C_{Y_{\dot{\beta}}} \right)  \\
-\frac{Sb}{\hat{c}} C_{l_\beta}  & \frac{Sb^2}{2\hat{c}} C_{l_p}   &  \frac{Sb^2}{2\hat{c}} \left( C_{l_r} - C_{l_{\dot{\beta}}} \right) \\
-\frac{Sb}{\hat{c}} C_{n_\beta}  & \frac{Sb^2}{2\hat{c}} C_{n_p}   &  \frac{Sb^2}{2\hat{c}} \left( C_{n_r} - C_{n_{\dot{\beta}}} \right) \\
\end{array}\right]
\label{eq:A1_coeff}
\end{equation}
%---------------------------------
% 
These matrices come from the interpretation of the work evaluated by the DLM, given unitary rigid input modes. %The sign are adjusted to match consequence of the different directions of the DLM and body reference systems. 
%
In  ${\bA}_1$ the coefficients on the third column feature derivatives with respect to both $r$ and $\dot{\beta}$: this is consequence of the fact that a rigid mode relative to yawing, when the flow direction is constant,  embeds both the rotational-induced inflow effect as well as the one relative to a change in sideslip angle.  
%
%\par 
%
%For $k=0$, and still within the quasi-steady approximation, it holds that $\bA_1 = \left. \frac{\ddi {\bA}}{\ddi \,  ik} \right|_{k=0}$, and $\bA_2 = \frac{1}{2} \left. \frac{\ddi^2 {\bA}}{\ddi \,  (ik)^2} \right|_{k=0}$. Matrices $\bA_1$ and $\bA_2$ can be evaluated with finite differences on DLM given \bA(ik). Notice how this justifies the terminology \emph{quasi-steady}. 
%
\par 
%
Within this approach, there is a clear interpretation of the GAF matrices in terms aerodynamic force coefficients, hence, is possible to assess the relevance of terms relative to unsteady effects (like $\dot{\beta}$). 
%The first step consist in identifying in the GAF matrices the unsteady terms of interest. 
%Focus is now on the contribution of $\dot{\beta}$.  
%
%\par 
%
Dutch roll eigenvalues are depicted in Figure~\ref{f:RL_RIGID_variousSTEADY} for analyses carried out retaining or not  $C_{n \dot{\beta}}$. 
%
%a progressively increasing number of unsteady terms. 
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/RL_RIGID_cnbetadoteffect.pdf}
	\caption{Effects of $C_{n \dot{\beta}}$ derivative on Dutch roll eigenvalue.}
	\label{f:RL_RIGID_variousSTEADY}
\end{figure}
%----------------------------|
%
It is apparent that contribution of other unsteady terms is small. 
%; and among them the derivatives with respect to $\dot{\beta}$ weight the most. \inred{More extensive analyses have been carried out in which each  , and are not reported here for the sake of brevity. Occhio alla deduzione logica}. 
%
%
\par 
%
The authors remark that the interpretation of the GAF matrices in terms of aerodynamic derivative coefficients, as shown in equation \ref{eq:A1_coeff} does not hold anymore when added states are considered, as it can be trivially verified recalling equation \ref{eq:Roger}. 
%
%In fact, with reference to equation , also higher order terms will contribute to the first derivative.}
%\inred{ remark how the term \emph{unsteady}
%
%one-to-one correspondence of the terms gand also given the DLM enables to augment the classic  give a one-to-one correspondence between the classic approach 
%
%
%There is however, a idiosyncrasy
%
%It is important to remark that this correspondence does not hold anymore when added states are considered. In fact, with reference to equation \ref{eq:Roger}, also higher order terms will contribute to the first derivative.}
%\inred{Discussione filosofica. Io determino A0 A1 ed A2 su tabulated data. I lag servono a migliorare il fitting, ma perderei il significato}  
%
\subsubsection{Importance of an appropriate RFA interpolation}
%
Expected outcome of RFA application is obtaining a good approximation of the  tabulated GAF coefficients given by the DLM keeping as low as possible the number of added aerodynamic states. 
In practice, it is important to have a reliable approximation in the frequency region of the phenomenon of interest.  
When studying the stability of the free-flying flexible aircraft, such phenomena span both low (almost zero)  and higher frequency range. 
%
For this reason, the modified Roger approach proves to be helpful in improving interpolation precision in the low frequency region. In fact, recalling from section \ref{s:FDDA}.\ref{ss:Aerodynamic}), modified Roger adds to the original set of least-square equations a further constraint for the derivative of the GAF matrix at zero frequency. 
% (, proves to be helpful to improve precision in the low frequency region. %quasi-steady region. 
This is shown in Figure~\ref{f:UFFD_6lag_21k_RogervsMod}, in which the $A_{1,3}$, is depicted for the Roger and Roger Mod methods. 
In the latter case the interpolation precision in the low frequency region is increased (at the expense, however, of the mid frequency one).
% 
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.75\textwidth]{./figures/UFFD_6lag_21k_RogervsMod.pdf}
	\caption{RFA with Roger and Roger Mod on 21 tabulated values. Value of GAF coefficient $A_{1,3}$.}
	\label{f:UFFD_6lag_21k_RogervsMod}
\end{figure}
%----------------------------|
%
It is true that RFA, in this case based on Roger's method, can be fine-tuned selecting the appropriate number of aerodynamic states, the frequencies to create the tabulated data and the values of the lag terms. 
It is also true that typical guidelines for flutter analysis can be retained, and accuracy can be further improved in the low frequency region just adding in the least square process the derivative (for example, evaluated at zero frequency).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                  %
\subsection{Flight dynamics considering the deformable aircraft}   %
%                                                                  %                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\label{ss:flexfd}
%
In this section the aircraft flexibility is taken into account. 
A system similar to the one of equations~\ref{eq:matrix_nolag} but  featuring also aerodynamic added states (full unsteady modeling of the aerodynamic forces) is solved for eigenvalues, hence, stability analysis. 
Other than the three rigid motions, 22 elastic modes have been included in the analysis~\cite{UC3Mteam_PrP1ceas}. 
Only Dutch roll eigenvalues are shown in Figure~\ref{f:DutchRoll_RigidvsElastic}.   
% 
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/DutchRoll_RigidvsElastic.pdf}
	\caption{Comparison of Dutch roll mode for rigid and flexible aircraft.}
	\label{f:DutchRoll_RigidvsElastic}
\end{figure}
%----------------------------|
%
Differences with the rigid vehicle case are remarkable. Table~\ref{tab:FQ_PrP} quantitatively reports this  difference at the cruise and sea level altitudes.  
%----------------------------
%     TABLE                 |
%----------------------------
\begin{table}[htp]
	\centering
	\begin{tabular}{c|c|c|c|c|}
		\cline{2-5}
		& \multicolumn{2}{c|}{Sea Level} & \multicolumn{2}{c|}{Cruise} \\ \cline{2-5} 
		& Rigid & Flexible & Rigid & Flexible \\ \hline
		\multicolumn{1}{|c|}{Eigenvalue} & $-0.1298 \pm 0.5586 i$ & $-0.08585 \pm 0.5584 i$ & $-0.08167 \pm 0.4102 i$ & $-0.05375 \pm 0.4063 i$ \\ \hline
		\multicolumn{1}{|c|}{$\omega_{nd}$ {[}$s^{-1}${]}} & 0.5735 & 0.5650 & 0.4183 & 0.4098 \\ \hline
		\multicolumn{1}{|c|}{$\zeta_d$} & 0.2263 & 0.1520 & 0.1953 & 0.1311 \\ \hline
	\end{tabular}
	\caption{Elastic aircraft: Dutch roll eigenvalue at sea level ($h = 0$ m and $V = 196$ m/s) and cruise ($h = 10500$ m and $V = 252$ m/s)}
	\label{tab:FQ_PrP}
\end{table}
%---------------------------
%
In terms of flying qualities, elasticity worsen aircraft behavior, inducing almost a drop to level 3, according to MIL-F-878C based Table~\ref{t:MILF}. 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                  %
\subsection{Aeroelasticity}   %
%                                                                  %                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The analysis performed in the previous section~\ref{ss:flexfd} gives as outputs all the eigenvalues of the system. 
Figure~\ref{f:UFFD_root locus_elastic} depicts the root locus considering only six elastic modes plus the Dutch roll mode. With aid of Figure~\ref{f:UFFD_elastic} it is possible to better quantify the flutter speed, occurring approximately at $V_\infty = 157$~m/s. 
% 
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/UFFD_rootlocus_elastic.pdf}
	\caption{Root locus for the free-flying elastic aircraft. Dutch roll and six first elastic modes eigenvalues plotted.}
	\label{f:UFFD_root locus_elastic}
\end{figure}
%----------------------------|
%
At this speed the first elastic mode becomes unstable. Frequency coalescence with the second elastic mode is observed as well. 
% 
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/UFFD_elastic.pdf}
	\caption{Real and imaginary parts of the eigenvalues at different speeds. Free-flying elastic aircraft.}
	\label{f:UFFD_elastic}
\end{figure}
%----------------------------|
%
As opposed to the longitudinal case, shown in efforts~\cite{SDSUteam_6jour,UC3Mteam_PrP1ceas}, where there was a clear interaction between the short period and the first two elastic modes that postponed flutter onset, here the picture is less clear. 
%
In fact, it is not evident if the drop in flutter speed compared to the fixed configuration case~\cite{SDSUteam_8scitech} is induced by the change in the free vibration properties of the system and/or by the interaction with the Dutch roll mode. 
%
\par 
%
For a more in-depth understanding, a comparison is carried out against the case in which aerodynamic coupling of the elastic and rigid modes is not taken into account. 
As it is apparent from the theoretical section~\ref{s:FDDA}, thanks to the assumptions carried throughout the derivation, the aerodynamic operator is the only one carrying all rigid/elastic coupling effects. % the rigid and elastic part is . 
With reference to system of equations~\ref{eq:matrix_nolag}, even though strictly valid only for the quasi-steady approximation, it can be appreciated how the terms $\bA_{i_{ER}}$ and $\bA_{i_{RE}}$ are the ones coupling the two dynamics. 
Selectively set them to zero will lead to uncoupled evolution of the rigid and elastic parts. 
%
%----------------------------
%     FIG                   |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=0.99\textwidth]{./figures/UFFD_elastic_coupl_uncoup.pdf}
	\caption{Aerodynamically coupled and uncoupled systems: real and imaginary parts of the eigenvalues at different speeds. Free-flying elastic aircraft. }
	\label{f:UFFD_elastic_coupl_uncoup}
\end{figure}
%----------------------------|
% 
\par 
%
Results of such comparison are shown in Figure~\ref{f:UFFD_elastic_coupl_uncoup}. 
It can be inferred that flutter speed slightly increases due to the elastic-rigid interaction. 
A previous work~\cite{SDSUteam_8scitech} showed, for the same aircraft (although slightly differently  modeled), large differences in flutter speed between free-flying and fixed-in-space models when antisymmetric behavior was investigated.  %in case of a free-flying and a clamped models. 
In view of the here-shown results, it can be argued that the low flutter speed does not depend on a detrimental aerodynamic interaction between rigid and elastic modes, but, simply on the different shape and frequency that elastic modes have with respect to the fixed-in-space model. 



==> chapters/V_Results_updated_lateral.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %
\subsection{Lateral-directional case}    %
%                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Dutch Roll and flying qualities}    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The comparison of the Dutch Roll for elastic and rigid vehicle at sea and cruise level is shown in Fig.~\ref{f:Dutch_roll_comparison}. 
It can be appreciated how considering the elastic interaction shifts the branch associated to the considered mode towards the imaginary axis, similarly as what seen for the Short Period. 
In this case, for the analysis at cruise level, Dutch Roll is unstable at low speeds, becoming stable at a speed of approximately 130 m/s. 
It is stressed out, anyway, that for the analysis, both compressibility correction and trim condition have been evaluated at cruise speeds only and, while results may be considered quantitatively valid around the linearization points, they only retain qualitative meaning far from them.
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Dutch_roll_comparison_comp}
	\caption{Comparison of Dutch roll mode for rigid and elastic vehicle at sea and cruise levels.}
	\label{f:Dutch_roll_comparison}
\end{figure}
%----------------------------|
%
%
\par
%
Requirements provided by the MIL-F-8785C for the Dutch Roll mode, for vehicles of class III, are based on three different levels of quality (1 is the best, 3 is sufficient) and on different flight phases, given by the categories. Constraints are given for minimum values of the damping ratio, frequency and their product (absolute value of the real part of the pole), assuming a stable Dutch Roll, as shown in Tab~\ref{t:MILF_lateral}.  
%
%----------------------------
%     TABLE                 |
%----------------------------
\begin{table}[!ht]
	\centering
	\begin{tabular}{ccccc}
		\hline\noalign{\smallskip}
		 \multicolumn{2}{l}{\textbf{Requirements}}  &  \\ 
		\noalign{\smallskip}\hline\noalign{\smallskip}
		\textbf{FQ Level} & \begin{tabular}[c]{@{}c@{}}\textbf{Flight Phase}\\ \textbf{Category}\end{tabular} & \multicolumn{1}{c}{\textbf{Min $\zeta_{d}$}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Min $\zeta_{d} \, \omega_{n_d}$}\\ \textbf{{[}rad/s{]}}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Min $\omega_{n_d}$}\\ \textbf{{[}rad/s{]}}\end{tabular}} \\
		\noalign{\smallskip}\hline\noalign{\smallskip}
		\multirow{3}{*}{1} & A & 0.19 & 0.35 & 0.4 \\
		& B & 0.08 & 0.15 & 0.4 \\
		& C & 0.08 & 0.10 & 0.4 \\ 
		\noalign{\smallskip}\hline\noalign{\smallskip}
		2 & All & 0.02 & 0.05 & 0.4 \\ 
		3 & All & 0.00 & 0.00 & 0.4 \\ 
		\hline\noalign{\smallskip}
	\end{tabular}
	\caption{Flying quality level requirements for Dutch Roll according to the MIL-F-8785C; aircraft of class III. Category B comprehends cruise.}
	\label{t:MILF_lateral}
\end{table}
%----------------------------
%
Tab.~\ref{t:dutch_roll_PrP250} shows the Dutch Roll eigenvalues for rigid and elastic cases both at sea level and cruise level. For sake of clarity, only values at cruise speeds for both the considered altitudes are reported. 
It can be appreciated that, for the rigid aircraft, at sea level, the current configuration fits into quality level 2. At cruise level, instead, it doesn't fit any of the three proposed levels, due to the limited value of the relative $\omega_{n_d}$. The elastic case reports a noticeable drop in the parameters associated to the pole damping ratio: notice a 51\% and a 92\% drop at sea and cruise level, respectively . At sea level, reduced absolute value of the real part of the pole, for the elastic case, almost induces a drop to quality level 3. At cruise level, the elastic configuration partially recovers Dutch Roll frequency without, although, being able to fit into quality level 3.
%------------------------------------------%
% TABLE Variables                  %
%------------------------------------------%
\begin{table}[!t]
\caption{Dutch Roll eigenvalues at sea and cruise levels for the PrP250. }
\label{t:dutch_roll_PrP250}       
\centering
\begin{tabular}{ c c c c c }
\hline\noalign{\smallskip}
&  \multicolumn{2}{c}{\textbf{Sea level}} &  \multicolumn{1}{c}{\textbf{Cruise}} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
& \textbf{Rigid} & \textbf{Elastic} & \textbf{Rigid} & \textbf{Elastic} \\
Eigenvalue                    & -0.1137 + i0.5335 & -0.0587 + i0.5487 & -0.0439 + i0.2552& -0.0037 + i0.2821\\
$\omega_{n_{d}} [s^{-1}]$     &0.52           & 0.55              & 0.25             & 0.2822 \\
$ \zeta_{d}$                  &0.2182         & 0.1064            & 0.17             &  0.013\\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}
%------------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Effect of DLM corrections on Dutch Roll mode}    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In this effort, for the first time, an enhanced DLM method is used to investigate the stability of a PrandtlPlane configuration. The extra terms included in the formulation consist in an enhanced boundary condition, which takes into account yaw-dihedral coupling, and a force calculation method which considers lateral loads and yawing moments due to roll rate and rolling moments due to yaw and yaw rate. 
%
\par
%
For this reason it is particularly interesting to asses the effects of such forces (ignored by a classic DLM formulation) on the stability of the Dutch Roll mode. Fig.~\ref{f:Dutch_roll_comparison} compares the Dutch Roll for the rigid and elastic configurations, at sea level, evaluated with UFFD by means of the classic and the enhanced DLM. 
It can be clearly seen how, for this aircraft configuration and for both the rigid and the elastic cases, the tendency of a more inclusive generalized force calculation procedure is to push the Dutch Roll mode at lower frequency and absolute value of the pole real part. 
In the perspective of flight quality assessment, then, the use of an enhanced DLM method may be decisive for the correct prediction of lateral-directional flight dynamics.
%In the perspective of flight quality assessment, then, the use of an enhanced DLM method may be decisive for the correct prediction of an acceptable or an unacceptable (or even unstable) Dutch roll mode. \inred{da rivedere periodo}
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Dutch_roll_correction_comparison}
	\caption{Comparison of Dutch Roll mode evaluated with classic and enhanced DLM for the rigid and elastic vehicle at sea level. }
	\label{f:Dutch_roll_comparison}
\end{figure}
%----------------------------|
%
%
%----------------------------
%     TABLE                 |
%----------------------------
\begin{table}[!ht]
\caption{Corrections in the aerodynamic matrices  $\widetilde{\bA}_{RR_0}$ and   $\widetilde{\bA}_{RR_1}$. Dimension is force per unit of dynamic pressure: [m$^2$]. Indexes are: 1 for translation along the span, 2 for roll, 3 for yaw.}
\label{t:enhanced_DLM coefficient} 
	\centering
	\begin{tabular}{lccccc}
		\hline\noalign{\smallskip}
		  & \textbf{Classic} & \textbf{Boundary Corr.} & \textbf{1st Term Corr.} &  \textbf{3rd Term Corr.} &  \textbf{All} \\
		\noalign{\smallskip}\hline\noalign{\smallskip}
		$\widetilde{\bA}_{0}^{13}$ &-108.0&-107.8&-100.2&-108.0&-100.0\\
		$\widetilde{\bA}_{0}^{23}$ &-228.8&-228.5&-259.2&-228.8&-258.7\\
		$\widetilde{\bA}_{0}^{33}$ &-329.8&-329.2&-290.6&-329.8&-290.1\\
		$\widetilde{\bA}_{1}^{12}$ &476&512&215&276&47\\
		$\widetilde{\bA}_{1}^{22}$ &-130550&-130722&-132207&-130550&-132354\\
		$\widetilde{\bA}_{1}^{32}$ &950&813&-7698&-4166&-12992\\
		\noalign{\smallskip}\hline
\end{tabular}
\end{table}
\inred{In Tab.Z\ref{t:enhanced_DLM coefficient} notice the change in sign $\widetilde{\bA}_{1}^{32}$. Turns out that it is mainly due to the presence of the fuselage in the fist term correction. Remember now we have a speed for a vertical panel (dihedral 1) which is not directed along the panel chord. The correction factor here is maximized.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Aeroelasticity}    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The unified analysis presented in the previous section (\emph{elastic} case) gives as outputs all the eigenvalues of the system. 
Fig.~\ref{f:Flutter_long} shows the complete lateral-directional stability analysis performed with UFFD in terms of frequency and damping coefficients of the system poles versus the asymptotic speed. Similarly to what done for the longitudinal case, the unified analysis of the free-flying configuration is compared with the flutter results of the cantilever wing system. 
It can be seen, for both the Cantilever and the Free-Flying case, a coalescence between the first two elastic modes. While, anyway, flutter occurs at a speed of approximately 270 m/s for the Cantilever configuration, for the Free-Flying one flutter point drops drastically to 155 m/s. In both cases the first elastic mode becomes unstable.
%
%
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Flutter_lateral_comp}
	\caption{PrP250 stability diagram for the lateral directional analysis: frequency and damping of the system at different speeds and sea level. Comparison between Cantilever and Free-Flying configurations.}
	\label{f:Flutter_long}
\end{figure}
%----------------------------|
%
\par
%
As opposed to the longitudinal case, where there is a clear interaction between the short period and the first elastic mode that postpones flutter onset, here the picture is less clear. 
%
It is not evident if the drop in flutter speed compared to the fixed configuration case is induced by the change in the free vibration properties of the system and/or by the interaction with the Dutch Roll mode. 
it is highlighted, in fact, the change in the free vibration mode frequencies of the syastem which can be inferred from the frequency diagram at asymptotic speeds close to zero.
%
\par 
%
For a more in-depth understanding, same as what already done for the longitudinal case, a comparison is carried out against the case in which aerodynamic coupling of the elastic and rigid modes is not taken into account. 
%
\par
%
Result of such comparison is shown in Figure~\ref{f:Flutter_lateral_uncoupled}. 
It can be inferred that flutter speed slightly increases due to the elastic-rigid interaction. 
A previous work~\cite{SDSUteam_8scitech} showed, for the same aircraft (although slightly differently  modeled), large differences in flutter speed between Free-Flying and fixed-in-space models, when anti-symmetric behavior was investigated.  %in case of a free-flying and a clamped models. 
In view of the here-shown results, it can be argued that the low flutter speed does not depend on a detrimental aerodynamic interaction between rigid and elastic modes, but, simply on the different shape and frequency that elastic modes have with respect to the fixed-in-space model. 
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Flutter_coupl_lateral}
	\caption{Free-flying elastic PrP250 stability diagram: frequency and damping of the system at different speeds and sea level. Comparison between coupled and uncoupled lateral-directional flight dynamics and aeroelasticity.}
	\label{f:Flutter_lateral_uncoupled}
\end{figure}
%----------------------------|
%

==> chapters/V_Results_updated_long.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
\inblue{In this section, results of the investigation relative to the response of the free-flying PrP250 aircraft are shown. First, the flying qualities are discussed, for both the longitudinal and lateral-directional dynamics; emphasis is given on effects of the enhanced DLM in the response prediction. 
Then, the aeroelastic view-point is adopted. Results for both longitudinal and lateral-directional dynamics are presented, and focus is on the physical sources of differences between  the case in which the aircraft is fixed  or free in the space. Again, importance of terms included in the enhanced DLM is discussed.}
%
%

%Previous studies using UFFD framework already assessed the influence of DLM-based unsteady aerodynamic terms in predicting the flight dynamics of the rigid aircraft for the longitudinal case~\cite{UC3Mteam_PrP1ceas} and lateral-directional one~\cite{UC3M_UFFDScitech}. They also pointed out the importance, for coupled analyses, to increase RFA accuracy on a wider range of frequencies due to the need of describe both flight dynamics and aeroelastic phenomena.
%
%\par
%
%In this effort, for both the longitudinal and lateral-directional planes, flying qualities of the studied configuration are evaluated for the rigid and the elastic cases and compared to the requirements provided by our reference: the MIL-F-8785C~\cite{SpecificationMILF}. 
%Such requirements involve the open loop system response to the pilot control and are expressed as constraints on the poles representing the flight dynamics of the vheicle.
%Focus is on how flying qualities are affected (and degradated) by taking into account structural flexibility. Moreover, for the current aircraft configuration, differences are shown, for the lateral-directional Dutch Roll mode, between using the traditional DLM or the enhanced one for the evaluation of aerodynamic forces.
%%and at what extent flight dynamic affects the aeroelastic response. 
%Finally, coupled analysis will focus on the occurrence of flutter instability.
%
%\par 
\subsection{Flight conditions and settings}
%
For this study, the aircraft is considered at straight-and-leveled flight. 
\inblue{Two conditions in the flight envelope are considered. Both refer to the aircraft at $V_C$, but at the different altitudes, namely, cruise altitude $h_c = 10500~m$ and sea level. 
At cruise altitude the Mach is $0.85$ (for a true airspeed of $V_\infty=252~m/s$). At sea level, the speed is $V_\infty=196~m/s$ (equivalent to a Mach number of approximately  $M=0.58$). 
%For both conditions, a weight equal to the MTOW has been considered.
}
%
\par
%

%Flying qualities are quantitatively assessed at sea level and nominal altitude cruise conditions, namely, $V_\infty=196~m/s$ at sea level, and  $V_\infty=252~m/s$ at an altitude of $10500~m$ (corresponding to a Mach number of 0.85). 
Compressibility correction, based on the Prandtl-Glauert rule, is used for aerodynamic calculations at cruise speed Mach number for both considered altitudes. 
%
\par
%
\inblue{For the analyses, in the case of flexible aircraft, 25 normal modes, three rigid  and 22 elastic for each case (longitudinal and lateral-directional) have proven to ensure convergence of results.}
%
\inblue{A set of tabulated GAFs is calculated on 21 reduced frequencies, chosen to cover the physics of interest; RFA is carried out on such data using 6 lag terms. RFA process followed a modified Roger method, as described in section \label{sss:rational}, to resolve accurately the dynamics for frequencies typical of both flight dynamics and aeroelastic phenomena.}
%
%
%RFA is performed for a set of 21 reduced frequencies, representative of the natural frequencies of the elastic modes used for the analyses. 
%
%Concerning stability analyses, for the elastic case, 25 structural modes are selected for the analysis (3 rigid modes and 22 elastic ones) which proved to ensure convergence of results. RFA is performed for a set of 21 reduced frequencies, representative of the natural frequencies of the elastic modes used for the analyses. 
%RFA is performed using Roger Mod method with 6 poles. 
%These settings proved to resolve successfully the dynamics for the range of frequencies interested by both the rigid modes and the elastic ones. 
\par%
\inblue{In the case of rigid aircraft the three rigid modes are trivially selected. In such case a quasi-steady approximation has been conveniently performed to correctly model Short Period and Dutch Roll modes.}
%
%
%
%For the rigid case, only 3 rigid modes are selected, number of reduced frequencies is 6 and no poles are selected for RFA (quasi-steady approximation of Sec.~\ref{sss:rational}) since the only dynamics to be caught is the one relative to the Short Period, concentrated in a very short range of frequencies~\cite{UC3Mteam_PrP1ceas}. 
%
\par
%
\inblue{It is stressed out that the enhanced DLM needs the evaluation of the aerodynamic flow properties (such as angle of attack and vortex circulation) in the reference flight conditions. Hence, for each flight condition a preliminary aerodynamic analysis with the VLM part embedded in the DLM is launched.}
%
%trim calculations for the evaluation of aerodynamic forces. Such conditions coincide with the speed above specified for the two considered altitudes.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                     %
%\subsection{Longitudinal case}                 %
\subsection{Flight dynamics of the flexible PrP}   
%                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\inblue{To assess handling qualities of the aircraft requirements provided by the MIL-F-8785C are referenced for the cases of Short Period and Dutch Roll. Such requirements relate a handling quality, ranging from 1 (best) to 3 (sufficient), to the eigenvalues properties such as damping ratio  and/or frequency. 
%
The numerical ranges that determine the handling quality, however, depend on the vehicle class and flight phase. 
The PrP250 is classified as aircraft of class III (\inred{[for his mass?]}). Being only considered cruise conditions,  the flight phase category is B.}
%
\par
%
\inblue{Both flying qualities for rigid and flexible aircraft are considered in order to assess effects of flexibility, for bot the longitudinal and lateral-directional dynamics.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Short Period and flying qualities}  %\label{s:short_period}  %
\subsubsection{Longitudinal case} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The comparison of the Short Period for elastic and rigid vehicle at sea level and cruise level is shown in Fig.~\ref{f:Short_period_comparison}.
%
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Short_period_comparison_comp}
	\caption{Comparison of Short Period mode for rigid and elastic vehicles at sea and cruise levels.}
	\label{f:Short_period_comparison}
\end{figure}
%----------------------------|
%
\inblue{It can be noticed how, as speed increases the elastic branch moves upward towards the imaginary axis to higher frequencies, for both cruise conditions. It will be shown in the following section how this behaviour is consequence of the interaction with elastic Mode I.}
%
\par
%
%Requirements provided by the MIL-F-8785C for the short-period are based on three different levels of flying qualities (1 is the best, 3 is sufficient). 
%The aircraft class and the chosen flight phase (given by the category) determine the specific values to be fulfilled by the aircraft as shown in Tab.~\ref{t:MIL_Short_period}.
%
\inblue{For the Short Period the MIL-F-8785C prescribes specific values on the damping ratio, as shown in  Tab.~\ref{t:MIL_Short_period} for a class III aircraft, like the PrP250, in cruise (Category B).}
%
%
%For vehicles of class III, like the PrP250, the chosen flight phase (given by the category) determines the specific values to be fulfilled by the aircraft as shown in Tab.~\ref{t:MIL_Short_period}.
%
%------------------------------------------%
% TABLE Variables                  %
%------------------------------------------%
\begin{table}[!t]
\caption{Flying quality requirements for Short Period damping ratio: aircraft of class III in cruise (category B).}
\label{t:MIL_Short_period}       
\centering
\begin{tabular}{c c}
\hline\noalign{\smallskip}
 \multicolumn{1}{l}{\textbf{Requirements}}  &  \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
 %\textbf{Categories A and C} & 
 \textbf{Category B} &  \textbf{Flying quality level}    \\ 
 \noalign{\smallskip}\hline\noalign{\smallskip}
  %$0.35 \leq \zeta_{SP} \leq 1.30$& 
  $0.30 \leq \zeta_{SP} \leq 2.00$& 1\\
  %$0.25 \leq \zeta_{SP} \leq 2.00$& 
  $0.20 \leq \zeta_{SP} \leq 2.00$& 2\\
  %$0.15 \leq \zeta_{SP}$ & 
  $0.15 \leq \zeta_{SP} $& 3\\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}
%------------------------------------------%
%
\inblue{Tab.\ref{t:short_period_PrP250} summarizes the values of damping ratio found for rigid and elastic aircraft.  %the study of the Short Period conducted with UFFD for both rigid and elastic cases at both sea level and cruise level. 
For the sake of clarity, only values of the poles for $V_C$ at both considered altitudes are shown.}
%
%Tab.\ref{t:short_period_PrP250} resumes the study of the Short Period conducted with UFFD for both rigid and elastic cases at both sea level and cruise level. For the sake of clarity, only values of the poles for the cruise speed at both considered altitudes are given. 
Comparing data in Tab.\ref{t:short_period_PrP250} with the requirements in Tab.~\ref{t:MIL_Short_period} it can be inferred that the considered configuration  fulfills the requirements for Flying quality level 1,  both for the rigid case and for the elastic one. 
%
It is worth to underline, however, the significant reduction of the $\zeta_{SP}$ when flexibility of the aircraft is considered, and namely, a $40\%$ and $32\%$ reduction at sea level and cruise altitude, respectively, which pushes the flying quality towards the lower boundary of level 1. 
%
%
This underline how, flexibility of the aircraft is a fundamental parameter to consider for the study of PrP250 flying qualities.
%
%given speeds) that reveals how the flexibility of the aircraft is a fundamental parameter to consider for the study of its flying qualities.
%
%------------------------------------------%
% TABLE Variables                  %
%------------------------------------------%
\begin{table}[!t]
\caption{Short Period eigenvalues at sea and cruise levels for the PrP250. }
\label{t:short_period_PrP250}       
\centering
\begin{tabular}{ c c c c c }
\hline\noalign{\smallskip}
&  \multicolumn{2}{c}{\textbf{Sea level}} &  \multicolumn{1}{c}{\textbf{Cruise}} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
& \textbf{Rigid} & \textbf{Elastic} & \textbf{Rigid} & \textbf{Elastic} \\
Eigenvalue & -1.31 + i0.93 & -1.23 + i2.40 & -0.69 + i1.00& -0.63 + i1.69\\
$\omega_{n_{SP}} [s^{-1}]$ &1.6 & 2.69& 1.21  & 1.80 \\
$ \zeta_{SP}$.         &0.82   & 0.45  & 0.57  &  0.35\\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}
%------------------------------------------%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Short Period and flying qualities}  %\label{s:short_period}  %
\subsubsection{Lateral-directional case} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Aeroelasticity}    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%After analysing the flight qualities related to the short-period mode
The unified analysis presented in the previous section (\emph{elastic} case) gives as outputs all the eigenvalues of the system and allows to identify the effects of mutual interaction between the flight dynamics and the aeroelastic behaviour of the configuration. Fig.~\ref{f:Flutter_long} shows the complete longitudinal stability analysis performed with UFFD on the test case in terms of frequency and damping coefficients of the system poles versus the asymptotic speed. Following the same strategy used in~\cite{SDSUteam_6jour,SDSUteam_8scitech} the unified analysis of the Free-Flying configuration is compared with the flutter results of the \emph{Cantilever} wing system~\cite{Divoux_tesi}. The comparison is able to highlight the different behaviours induced by the presence of the rigid modes on the flutter response. Differently than previous studies, this time the fully unified model takes into account the vehicle flight dynamics and the rigid pitching mode assumes the meaning of a Short Period. As seen from Fig. 13, for the cantilever configuration flutter occurs at approximately 281 m/s while the free-flying configuration is flutter free in the considered speed range, up to 300 m/s. This confirms the trend seen in~\cite{SDSUteam_6jour} where, in the given interpretation, considering the fuselage inertial properties, the Short Period mode interacts with the first elastic mode, postponing the coalescence of the first two elastic modes responsible of flutter occurrence.
%
\par
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Flutter_long_comp}
	\caption{PrP250 stability diagram for the longitudinal analysis: frequency and damping of the system at different speeds and sea level. Comparison between Cantilever and Free-Flying configurations.}
	\label{f:Flutter_long}
\end{figure}
%----------------------------|
%
In order to endorse such interpretation, a comparison is carried out against the case in which the aerodynamic coupling between elastic and rigid modes is not taken into account. 
%
%As it is apparent from the theoretical section~\ref{s:FDDA}, thanks to the assumptions carried throughout the derivation, the aerodynamic operator is the only one carrying all rigid/elastic coupling effects. 
%With reference to system of equations~\ref{eq:matrix_nolag}, even though strictly valid only for the quasi-steady approximation, it can be appreciated how the terms $\bA_{i_{ER}}$ and $\bA_{i_{RE}}$ are the ones coupling the two dynamics. 
%Selectively set them to zero will lead to uncoupled evolution of the rigid and elastic parts. 
It is recalled, in fact, that, for the employed model, the only coupling contributions between the rigid and elastic equations of motion are given by the aerodynamic forces. Selectively setting $\bA_{i_{RE}}$ and $\bA_{i_{ER}}$ to zero (as shown in Eq.~\ref{eq:aero_coupling} in section~\ref{sss:flexible_aerodynamics}) leads to decouple the dynamics of the rigid aircraft and its aeroelastic behaviour. 
%
Results of such comparison is shown in Fig.~\ref{f:Flutter_long_uncoupled} where the stability analyses for the coupled and the uncoupled systems are compared. It can be seen how, for the uncoupled analysis, the Short Period mode doesn't interact with the first elastic one, partially recovering the trend observed for the cantilever analysis of Fig.~\ref{f:Flutter_long}, and flutter speed is anticipated. 
Nevertheless, flutter speed is still different from the one of the cantilever configuration. This is due to the fact that the two considered configurations exhibit different free vibration properties (shape and frequency of structural modes). It can be concluded that the raise in flutter speed observed for the free flying configuration is due to the synergistic effect of the change in the structural properties of the wing system \emph{and} the effect of the interaction with the Short Period mode.
%----------------------------
%     FIG       |
%----------------------------
\begin{figure}[htb]
	\centering
	\includegraphics[width=\textwidth]{./figures/Long_uncoupled_comp}
	\caption{Free-flying elastic PrP250 stability diagram: frequency and damping of the system at different speeds and sea level. Comparison between coupled and uncoupled longitudinal flight dynamics and aeroelasticity.}
	\label{f:Flutter_long_uncoupled}
\end{figure}
%----------------------------|
%


==> definition/boldmath.tex <==
% ********** WARNING  ************
% Use either this file boldmath.tex or file mathbf.tex, BUT NOT BOTH!!!

% Latin lowercase letters
\newcommand{\ba}{\boldmath{a}}
\newcommand{\bb}{\boldmath{b}}
\newcommand{\bc}{\boldmath{c}}
\newcommand{\bd}{\boldmath{d}}
\newcommand{\bes}{\boldmath{e}}     % special
\newcommand{\bef}{\boldmath{f}}     % special
\newcommand{\bg}{\boldmath{g}}
\newcommand{\bh}{\boldmath{h}}

\newcommand{\bi}{\boldmath{i}}     % versori
\newcommand{\bj}{\boldmath{j}}
\newcommand{\bk}{\boldmath{k}}

\newcommand{\bl}{\boldmath{l}}
\newcommand{\bm}{\boldmath{m}}      %
\newcommand{\bn}{\boldmath{n}}      % versore normale

\newcommand{\bp}{\boldmath{p}}
\newcommand{\bq}{\boldmath{q}}      % coord. di Lagrange
\newcommand{\br}{\boldmath{r}}
\newcommand{\bs}{\boldmath{s}}
\newcommand{\bt}{\boldmath{t}}
\newcommand{\bu}{\boldmath{u}}
\newcommand{\bv}{\boldmath{v}}
\newcommand{\bw}{\boldmath{w}}
\newcommand{\bx}{\boldmath{x}}     %%% Vettori
\newcommand{\by}{\boldmath{y}}
\newcommand{\bz}{\boldmath{z}}

% Uppercase letters
\newcommand{\bA}{\boldmath{A}}     %%% Matrici
\newcommand{\bB}{\boldmath{B}}
\newcommand{\bC}{\boldmath{C}}
\newcommand{\bD}{\boldmath{D}}
\newcommand{\bE}{\boldmath{E}}
\newcommand{\bF}{\boldmath{F}}      %
\newcommand{\bG}{\boldmath{G}}
\newcommand{\bH}{\boldmath{H}}
\newcommand{\bI}{\boldmath{I}}
\newcommand{\bJ}{\boldmath{J}}
\newcommand{\bK}{\boldmath{K}}
\newcommand{\bL}{\boldmath{L}}
\newcommand{\bM}{\boldmath{M}}
\newcommand{\bN}{\boldmath{N}}

\newcommand{\bP}{\boldmath{P}}
\newcommand{\bQ}{\boldmath{Q}}
\newcommand{\bR}{\boldmath{R}}
\newcommand{\bS}{\boldmath{S}}
\newcommand{\bT}{\boldmath{T}}
\newcommand{\bU}{\boldmath{U}}
\newcommand{\bV}{\boldmath{V}}      %  velocita'
\newcommand{\bW}{\boldmath{W}}
\newcommand{\bX}{\boldmath{X}}
\newcommand{\bY}{\boldmath{Y}}
\newcommand{\bZ}{\boldmath{Z}}

% Zero
\newcommand{\bzero}{\boldmath{0}}


==> definition/boldsymbol.tex <==
% ********** WARNING  ************
% Use either this file boldsymbol.tex or file mathbf.tex, BUT NOT BOTH!!!

% Latin lowercase letters
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bes}{\boldsymbol{e}}     % special
\newcommand{\bef}{\boldsymbol{f}}     % special
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}

\newcommand{\bi}{\boldsymbol{i}}     % versori
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}

\newcommand{\bl}{\boldsymbol{l}}
%\newcommand{\bm}{\boldsymbol{m}}      %
\newcommand{\bn}{\boldsymbol{n}}      % versore normale

\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}      % coord. di Lagrange
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}     %%% Vettori
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

% Uppercase letters
\newcommand{\bA}{\boldsymbol{A}}     %%% Matrici
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}      %
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}

\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}      %  velocita'
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

% Zero
\newcommand{\bzero}{\boldsymbol{0}}


==> definition/definiz.tex <==
%  File DEFINIZ.TEX
%
%% This file contains several macros that proved to be useful in some papers.
%% Use the command \input{definiz} in the preamble of your LaTeX file.

%% Definition of boldface letters, vectors, etc.:
%
  \def\reale{\mbox{I\kern-0.2em R}}  % Symbol for the set of real numbers.
%
  \def\bx{{\bf x}}                                                              
  \def\by{{\bf y}}
%
  \def\vn{\vec{n}}
  \def\ut{\tilde{u}}
%
  \def\bxi{\mbox{\boldmath $\xi$}}
  \def\bta{\mbox{\boldmath $\eta$}}
%
  \def\h{{\it h\/}}  %  Italics for h-hierarchical
  \def\p{{\it p\/}}
%
%% Shorts for Greek letters and other symbols
  \def\al{\alpha}
  \def\ep{\varepsilon}
  \def\th{\theta}
  \def\la{\lambda}
  \def\be{\beta}
  \def\de{\delta}
  \def\ga{\gamma}
  \def\La{\Lambda}
  \def\Om{\Omega}
  \def\Ga{\Gamma}
  %
  \def\pd{\partial}
  \def\lapl{\nabla^2}
  \def\at{\bigg|} % serve per dire dove va valutata una derivata.
  \def\sgn{\mathop{\rm sgn}} % funzione ``segno di''
%
%% Macros
%
  \newcommand{\sez}[1]{\section*{
			\protect\Large\sc\centering #1}} %% titolo sez.
						    %% centrato in \sc
  \newcommand{\subsez}[1]{\subsection*{\protect\large\it #1}}  %% subsez. it.
%
% Pedici in roman etc.
  \def\tr{t_{\mbox{{\scriptsize{ref}}}}}
  \def\dr{d_{\mbox{{\scriptsize{ref}}}}}
  \def\xln{\bar{\xi}_\la^n}
  %
  \def\Ll{{\varepsilon \to 0^{+}}}
  \def\limite{\lim_\Ll}
  %
  \def\T{T^{\omega}_{ij}}
  \def\U{U^{\omega}_{ij}}
%

%
%% Double integrals for 3D singular integrals.
  \def\dbint{\int_0^{2\pi}
	   \int_{\alpha(\varepsilon,\theta)}^{\hat{\rho}(\theta)}}
%                                                                               
  \def\dbintm{\int_{\th_1^m}^{\th_2^m}
	    \int_{\alpha^m(\varepsilon,\theta)}^{{\hat{\rho}}^m(\theta)}}
%
  \def\dbintn{\int_{\th_1^m}^{\th_2^m} \int_{0}^{{\hat{\rho}}^m(\theta)}}
%

%
%% Cauchy Principal Value and Finite Part Integrals
 \newlength{\meno}
 \newlength{\integrale}
 \newlength{\trattino}
 \newlength{\integralegrande}
 \newlength{\uguale}
 \newlength{\ugualegrande}
%
 \settowidth{\trattino}{\mbox{\large{-}}}
% \settowidth{\trattino}{\mbox{\tiny{--}}}
 \settowidth{\meno}{\mbox{$-$}}
% \settowidth{\uguale}{\mbox{$=$}}
 \settowidth{\uguale}{\mbox{\tiny{$=$}}}
 \settowidth{\ugualegrande}{\mbox{$=$}}
 \settowidth{\integrale}{\mbox{$\int$}}
 \settowidth{\integralegrande}{\mbox{$\displaystyle\int$}}
%
 \addtolength{\trattino}{\integrale}
 \addtolength{\meno}{\integralegrande}
 \addtolength{\uguale}{\integrale}
 \addtolength{\ugualegrande}{\integralegrande}
%

% definiz. degli integrali CPV e FP, sia piccoli che grandi.
%
 \newcommand{\FP}[2]{\mbox{\raisebox{0.17\integrale}{\tiny{$=$}}}%
		\mbox{\hspace{-0.5\uguale}}\mbox{$\int_{#1}^{#2}$}}
%
 \newcommand{\CPV}[2]{\mbox{\raisebox{-0.05\integrale}{\large{-}}}%
		\mbox{\hspace{-0.52\trattino}}\mbox{$\int_{#1}^{#2}$}}
%
 \newcommand{\CPVG}[2]{\mbox{$-$}\mbox{\hspace{-0.5\meno}}\mbox{$
				  \displaystyle\int_{#1}^{#2}$}}
%
 \newcommand{\FPG}[2]{\mbox{$=$}\mbox{\hspace{-0.5\ugualegrande}}\mbox{$
				  \displaystyle\int_{#1}^{#2}$}}
%

%% Shorts for commands.
  \newcommand{\bib}[1]{\bibitem{#1}}
%
  \def\beq{\begin{equation}}
  \def\eeq{\end{equation}}
%

%% ``Poor-man boldface'', useful for bold subscripts of Greek letters (see
%   The TeXbook)
  \def\pmb#1{\setbox0=\hbox{#1}%
  \kern-.025em\copy0\kern-\wd0
  \kern.05em\copy0\kern-\wd0
  \kern-.025em\raise.0433em\box0 }
% Example:  \pmb{$\scriptstyle \xi$}
%
% Commands to draw BEM pictures.
%
  \newcommand{\punto}[2]{\put(#1,#2){\circle*{1.5}}}  %nodo per BEM
  \newcommand{\vertic}[3]{\put(#1,#2){\line(0,1){#3}}} %linea verticale.
  \newcommand{\orizzo}[3]{\put(#1,#2){\line(1,0){#3}}} %linea orizzontale
  \newcommand{\prl}{\protect\large} %per le scritte
%
%%%
%
%  ``eqnarray'' with proper spacing around = sign
%  This new environment is called ``myeqnarray''
%
  \newenvironment{myeqnarray}{ %
  \protect\setlength{\arraycolsep}{0.14em} %%   0.14em = 2.5/18 quad = 0.5 thickspace,
 \begin{eqnarray} }{ %%%                default value was 5 pt (much bigger)
 \end{eqnarray} \kern-0.5em} %% see The TeXbook, p. 167-170 and p.60,76.
%


%%% New list with letters instead of numbers
%
   \newenvironment{alfabeto}{%
   \renewcommand{\theenumi}{\alph{enumi}}
   \renewcommand{\labelenumi}{\theenumi)}
   \begin{enumerate}	 }{%
   \end{enumerate}	  }

% Nota sulla prima pagina per dare informazioni sulla sede di pubblicazione
%
%% Footnote on the first page %%
 \newcommand{\sedepubblicazione}[1]{%
   \begin{table}[b]       % e` una tabella in fondo alla pagina.
     \footnotesize
     \footnoterule        % tratto di separazione
    {#1}                  % testo della nota
    \end{table}
  }                       % fine definizione


\def\azzera{\vspace{-\the\pagetotal}}	% riposiziona "quasi"
					%  all'inizio della pagina


==> definition/dotted.tex <==
% Dotted letters

\newcommand{\dbq}{\dot{\bq}}
\newcommand{\dbw}{\dot{\bw}}
\newcommand{\dbx}{\dot{\bx}}     %%% derivate temporali

\newcommand{\ddbq}{\ddot{\bq}}
\newcommand{\ddbw}{\ddot{\bw}}
%%\newcommand{\dbx}{\mathbf{\dot{x}}}  % NON sono uguali
\newcommand{\ddbx}{\ddot{\bx}}

\newcommand{\dg}{\dot{g}}
\newcommand{\dep}{\dot{p}}
\newcommand{\dq}{\dot{q}}


\newcommand{\dr}{\dot{r}}
\newcommand{\ds}{\dot{s}}
\newcommand{\du}{\dot{u}}
\newcommand{\dv}{\dot{v}}
\newcommand{\dw}{\dot{w}}
\newcommand{\dx}{\dot{x}}
\newcommand{\dy}{\dot{y}}
\newcommand{\dz}{\dot{z}}

\newcommand{\ddx}{\ddot{x}}
\newcommand{\ddy}{\ddot{y}}
\newcommand{\ddz}{\ddot{z}}


\newcommand{\dR}{\dot{R}}
\newcommand{\dH}{\dot{H}}
\newcommand{\dS}{\dot{S}}
\newcommand{\dF}{\dot{F}}
\newcommand{\dB}{\dot{B}}

\newcommand{\dbC}{\dot{\bC}} 
\newcommand{\ddbC}{\ddot{\bC}}

==> definition/margini.tex <==
% File margini.tex
%
% Page settings for A4 paper (21 x 29.7 cm):
%
  \topmargin  0pt	  % default: 27 pt = 0.95 cm  (1 pt = 0.352 mm)
  \headheight 0pt	  % def.   : 12 pt
  \headsep    0pt	  % def.   : 25 pt
  \textheight 24.0 cm	  %%%	excluding the head and the foot
%
  \oddsidemargin 0.0 cm   %%% 63, 54, 39.5 pt for styles 10,11,12 pt, resp.
  \textwidth 16.0 cm	  %%% 345,360,390 pt  "    "	    "          "
%
% Con questi valori di \topmargin e \oddsidemargin, si ha un bordo
% di 1 inch = 25.4 mm.
%%
%


==> definition/mathsf.tex <==
% San serif lowercase letters
\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathbf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}

\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}

% Sans serif uppercase letters

\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

% Zero
\newcommand{\sfzero}{\mathsf{0}}


==> definition/varie.tex <==
\newcommand{\lisi}[2]{$#1$ \> #2; \\}  % per lista dei simboli con tabbing

% From Johannes Braams:
%\addto\captionsitalian{\def\figurename{\textsf{Fig.\ }}}  % OLD
%\addto\captionsitalian{\def\figurename{\sffamily Fig.\ }} % NEW
\newcommand{\paginacorta}{\enlargethispage{-\baselineskip}}
\newcommand{\paginalunga}{\enlargethispage{\baselineskip}}
\newcommand{\paginacortissima}{\enlargethispage{-2\baselineskip}}
\newcommand{\paginalunghissima}{\enlargethispage{2\baselineskip}}
% Comandi per dare maggior liberta' nel posizionare le figure.
\renewcommand{\topfraction}{0.95}     % era 0.7   vedi book.cls
\renewcommand{\bottomfraction}{0.7}  % era 0.3
\renewcommand{\textfraction}{0.05}    % era 0.2
%  \newlength{\largh}{\textwidth} % si usa per la larghezza dei disegni .eps

%\newcommand{\e}{\operatorname{e}}  %% esponenziale
%% I seguenti comandi sono stati commentati perche' gia' esistono nelle
%% versioni piu' recenti di amslatex (o qualcosa di simile).
%% \newcommand{\tr}{\operatorname{tr}}  %% traccia
%% \newcommand{\dd}{\text{{\sl d}}}    %% differenziale
%% \newcommand{\grad}{\operatorname{grad}} %% gradiente
%% \newcommand{\rot}{\operatorname{rot}}   %% rotore
%\renewcommand{\div}{\operatorname{div}}


\newcommand{\Ind}[1]{#1\index{#1}}              % voce normale
\newcommand{\Indbf}[1]{#1\index{#1|textbf}}     % pagina in grassetto

\newcommand{\cedpage}{\newpage{\thispagestyle{empty}\cleardoublepage}}

